Unprovability of Strong Complexity Lower Bounds in Bounded Arithmetic

While there has been progress in establishing the unprovability of complexity statements in lower fragments of bounded arithmetic, understanding the limits of Je\v{r}\'abek's theory $APC_1$ (2007) and of higher levels of Buss's hierarchy $S^i_2$ (1986) has been a more elusive task. Even in the more restricted setting of Cook's theory PV (1975), known results often rely on a less natural formalization that encodes a complexity statement using a collection of sentences instead of a single sentence. This is done to reduce the quantifier complexity of the resulting sentences so that standard witnessing results can be invoked. In this work, we establish unprovability results for stronger theories and for sentences of higher quantifier complexity. In particular, we unconditionally show that $APC_1$ cannot prove strong complexity lower bounds separating the third level of the polynomial hierarchy. In more detail, we consider non-uniform average-case separations, and establish that $APC_1$ cannot prove a sentence stating that $\forall n \ge n_0\;\exists\,f_n \in \Pi_{3}$-$SIZE[n^d]$ that is $(1/n)$-far from every $\Sigma_{3}$-$SIZE[2^{n^{\delta}}]$ circuit. This is a consequence of a much more general result showing that, for every $i \geq 1$, strong separations for $\Pi_{i}$-$SIZE[poly(n)]$ versus $\Sigma_{i}$-$SIZE[2^{n^{\Omega(1)}}]$ cannot be proved in the theory $T_{PV}^i$ consisting of all true $\forall \Sigma^b_{i-1}$-sentences in the language of Cook's theory PV. Our argument employs a convenient game-theoretic witnessing result that can be applied to sentences of arbitrary quantifier complexity. We combine it with extensions of a technique introduced by Kraj\'i\v{c}ek (2011) that was recently employed by Pich and Santhanam (2021) to establish the unprovability of lower bounds in PV (i.e., the case $i=1$ above, but under a weaker formalization) and in a fragment of $APC_1$.

==> dialectica.tex <==

\section{On Witnessing via the Dialectica Interpretation}

We can use the Dialectica interpretation of first-order arithmetic to extract a witnessing theorem. To do this there are two steps. We firstly need to embedding classical first-order logic into intuitionistic first-order logic by double-negation translation. After that, we apply the Dialectica interpretation. 

Let $\varphi=\exists y_1\forall x_1\dots\exists y_k\forall x_k\phi(x,y_1,\dots,y_k,x_1,\dots,x_k)$ be a formula. Let $\tilde{\phi}$ be the double-negation translation of $\phi$, then the translation of $\varphi$ becomes
\begin{equation}\label{equ:double-negation}
\lnot\forall y_1\lnot \forall x_1\lnot \forall y_2\lnot \dots\lnot \forall y_k\lnot \forall x_k\lnot \tilde{\phi}.
\end{equation}
The Dialectica interpretation $(\cdot)^D$ for $\{\forall,\lnot\}$ is defined as follows. Let $\alpha^D=\exists x~\forall y~\alpha_D(x,y)$. 
\begin{enumerate}
\item $(\forall z~\alpha(z))^D\triangleq\exists X~\forall z,y~\alpha_D(X(z),y,z)$. The intuition is that the truthifier has a strategy $X$ to choose the strategy $x$ for the Dialectica game of $\alpha_D$ given any choice $z$ of the falsifier. 
\item $(\lnot\alpha)\triangleq\exists Y~\forall x~\lnot\alpha_D(x,Y(x))$. The intuition is that the negation switches players. There is a function $Y$ such that given any strategy $x$ for the truthifier in the Dialectica game of $\alpha_D(x,y)$, we can obtain a strategy $Y(x)$ for the falsifier in the Dialectica game of $\alpha_D(x,y)$ that beats the strategy $x$ for the truthifier. 
\end{enumerate}

We now read the equation (\ref{equ:double-negation}) using the Dialectica interpretation. Let $\alpha^D=\exists x~\forall y~\alpha_D(x,y)$. We can see that:
\begin{enumerate}[itemsep=0pt]
\item $(\lnot\forall z~\alpha)^D=\exists Y_1~\forall X_1~\lnot\alpha_D$, where: $X_1$ takes $z$ as input and produces the truthifier strategy for $\alpha_D$; $Y_1$ takes $X_1$ as input and produces the falsifier strategy for $\alpha_D$. 
\item $(\lnot \forall w~\lnot\forall z~\alpha)^D=\exists Y_2~\forall X_2~\lnot\alpha_D$, where: $X_2$ takes $w$ as input and produces $Y_1$ in (1); $Y_2$ takes $X_2$ as input and produces the $X_1$ in (1). 
\end{enumerate}
Now let $\phi_D$ be the Dialectica interpretation of $\lnot\tilde{\phi}$. 

==> model-theoretic-KPT.tex <==

\subsection{Model-theoretic proof of the KPT witnessing theorem for $\forall\exists\forall\exists$ sentences}
\label{sec:proof-of-four-quantifiers}

\begin{reminder}[\Cref{thm:KPT4}] Let $\calT$ be a universal theory with vocabulary $\calL$. Let $\varphi$ be a quantifier-free $\mathcal{L}$-formula, and suppose that $\mathcal{T} \;\vdash\; \forall x\, \exists y \, \forall z \, \exists w\;\varphi(x,y,z,w)$. Then there is a constant $\ell\ge 1$ and a sequence $t_1, \dots, t_k$ of $\calL$-terms such that
\[
\mathcal{T} \;\vdash\;  \forall x,z_1,\dots,z_k\;
\bigl(\psi(z,t_1(z),z_1) \lor \psi(x,t_2(x,z_1),z_2) \lor \dots \lor \psi(x,t_k(z_1,\dots,z_{k-1}),z_k)\bigr),
\]
where $\psi(x,y,z) \triangleq \exists w\,\varphi(x,y,z,w)$.
\end{reminder}


\begin{proof} We verify that an argument described in \citep[Section VIII.6]{cook_nguyen_2010} for the case of three quantifiers extends to sentences of this form.
Let $b, c_1, c_2, \ldots$ be a list of new constant symbols, and let $u_1, u_2, \ldots$ be an enumeration of all terms built from the functions and constants in $\mathcal{L}$ together with $b, c_1, c_2, \ldots$, where the only new constant symbols appearing in $u_k$ are among $b, c_1, \ldots, c_{k-1}$. 

For convenience, let $\psi(x,y,z) \eqdef \exists w\, \varphi(x,y,z,w)$, as in the statement of the theorem. We will argue that there exists a constant $k \geq 1$ such that no model  of $\mathcal{T}$ satisfies the sentence
$$
\neg \psi(b,u_1,c_1) \wedge \neg \psi(b,u_2,c_2) \wedge \ldots \wedge \neg \psi(b,u_k,c_k)\;.
$$
This implies that every model of $\mathcal{T}$ satisfies the negation of this sentence, and by the completeness theorem,
$$
\mathcal{T} \;\vdash\; \psi(b,u_1,c_1) \vee  \psi(b,u_2,c_2) \vee \ldots \vee  \psi(b,u_k,c_k)\;.
$$
Since $b, c_1, c_2, \ldots$ are new constants and each  term $u_k$ depends only on $b, c_1, \ldots, c_{k-1}$ (among the new constant symbols), the result follows.

To show the remaining claim, we argue by contradiction. Suppose that no finite $k$ satisfies the claim. Then, by compactness, we get that
$$
\mathcal{T} \cup \{\neg \psi(b,u_1,c_1), \neg \psi(b,u_2,c_2), \neg \psi(b,u_3,c_3), \ldots\}
$$
admits a model $\mathcal{M}$. Consequently,  using the definition of $\psi$,
$$
\mathcal{M} \;\models\;  \mathcal{T} \cup \{\forall w \,\neg \varphi(b, u_1, c_1, w),\; \forall w \,\neg \varphi(b, u_2, c_2, w), \ldots\}
$$
Let $\mathcal{T}^+ \eqdef \mathcal{T} \cup \{\forall w \,\neg \varphi(b, u_1, c_1, w), \forall w \,\neg \varphi(b, u_2, c_2, w), \ldots\}$. Since $\mathcal{T}$ is a universal theory and $\varphi$ is an open formula, it follows that $\mathcal{T}^+$ is also a universal theory. For this reason, the substructure $\mathcal{M}'$ of $\mathcal{M}$ consisting of the denotations of the terms $u_1, u_2, \ldots$ (under $\mathcal{M}$) is also a model of $\mathcal{T}^+$. Now it is not hard to prove that 
$$
\mathcal{M}' \;\models\; \mathcal{T} \;+\; \exists x\, \forall y\, \exists z\, \forall w\; \neg \varphi(x,y,z,w)\;,
$$
which contradicts the hypothesis of the theorem and completes the proof.
To see this, it is enough to show that $\mathcal{M'} \models \forall y\, \exists z\, \forall w \; \neg \varphi(b^{\mathcal{M}'},y,z,w)$. Given an arbitrary element $m$ of $\mathcal{M}'$, by construction of $\mathcal{M}'$, there is some term $u_k$ such that $m = u_k^{\mathcal{M}'}(b^{\mathcal{M}'}, c_1^{\mathcal{M'}}, \ldots, c_{k-1}^{\mathcal{M'}})$. Since $\mathcal{M}'$ is a model of $\mathcal{T}^+$, which includes the sentence $\forall w \,\neg \varphi(b,u_k,c_k,w)$, we get that $\mathcal{M}' \models \forall w\, \neg \varphi(b^{\mathcal{M}'}, m, c_k^{\mathcal{M}'}, w)$. This finishes the proof that  $\mathcal{M'} \models \forall y\, \exists z\, \forall w \; \neg \varphi(b^{\mathcal{M}'},y,z,w)$. 
\end{proof}








==> proof-overviews.tex <==
\section{Overview of the Proofs of \Cref{thm:intro_main_unprov} and \Cref{thm:intro_witnessing-tree-exploration}}
\label{sec:proof-overviews}






In this section, we provide a more detailed overview of our proofs. Since the game-theoretic witnessing result (\Cref{thm:intro_witnessing-tree-exploration}) is a key ingredient when showing the unprovability of strong complexity lower bounds in bounded arithmetic (\Cref{thm:intro_main_unprov}), we start off with a discussion of the former. 


\subsection{Game-theoretic witnessing for general formulas}

Let $\calT$ be a universal theory, and let $\varphi(x)$ be a formula with $x$ being the only free variable. Suppose that  $\calT\vdash\forall x~\varphi(x)$. The purpose of the witnessing theorem is to extract computational information from the provability of $\forall x~\varphi(x)$ that relates to the sentence $\varphi$. Without loss of generality, we work with the connectives $\{\to,\perp\}$ and define other connectives with them. 

\paragraph{Preliminaries of Proof Theory.} Recall that there are two equivalent interpretations of the statement $\calT\vdash\forall x~\varphi(x)$: the model-theoretic interpretation meaning that for every first-order model in which every axiom in $\calT$ is true, $\forall x~\varphi(x)$ is also true; and the proof-theoretic interpretation meaning that in some sound and complete proof system for the first-order logic, there is a proof of the sentence $\forall x~\varphi(x)$ from the axioms in $\calT$. In this work, we will use a proof-theoretic approach to extract information from a proof, and in particular, we will work with a variant of Gentzen's cut-free sequent calculus called $\GG$ (see, e.g., \cite{basic-proof-theory}). 

We start by presenting the definition and intuition of the proof system $\GG$. A \emph{sequent} is defined as $\Gamma\To\Delta$, where $\Gamma$ (called the \emph{antecedent}) and $\Delta$ (called the \emph{succedent}) are multisets of formulas. The sequent is interpreted as $\bigwedge\Gamma\to\bigvee\Delta$, i.e., assuming that all the formulas in $\Gamma$ hold, then at least one of the formulas in $\Delta$ is true. A \emph{proof tree} in $\GG$ is a tree of sequents with the conclusion on its root such that each node is a consequence of its child(ren) from one of the \emph{inference rules} (see \Cref{sec:cut-free-g3c}). By the completeness of $\GG$, we know that $\calT\vdash\forall x~\varphi(x)$ if and only if there is a proof tree that concludes $\Gamma\To\varphi(x)$, where $\Gamma\subseteq\calT$ is some finite subset of $\varphi(x)$. 

\paragraph{A Proof Search View of $\GG$.} Instead of viewing a proof tree as a derivation following the axioms, we can also treat it as a transcript of a \emph{proof search} procedure, which starts from the conclusion (i.e.~the root) as the goal, resolves goals and generates subgoals according to \emph{proof search rules} (i.e.~growing the tree reversely via inference rules), and terminates when all the (sub)goals are closed (i.e.~ending with axioms on the leaves). We now describe a proof search procedure that is essentially equivalent to $\GG$ proofs.


The proof search for a goal $S:\Gamma\To\Delta$ is defined as a recursive procedure: We pick one of the formulas $\psi$ (called \emph{principal formula}) in $S$ and apply the corresponding rule as follows, based on its outermost connective (or quantifier) and its position in the sequent $S$.\footnote{Note that in rule (Ax), the principal formula appears in both the antecedent and the succedent.}

\inote{What exactly is the goal of the proof search? How to decide what will be the principal formula? How does it affect the goal? Make sure the reader knows the rules of the game.}

\begin{description}[itemsep=0pt]\small
    \item[\footnotesize(Ax).] Assume that $S:\Gamma,P\To\Delta,P$ and the principal formula is one of these displayed $P$, and $P$ is of the form $R(t_1,\dots,t_k)$ for some relation symbol $R$ and terms $t_1,\dots,t_k$. In this case, the proof search terminates successfully.  
    \item[\footnotesize(L$\perp$).] If $S:\Gamma,\perp\ \To\Delta$ and the principal formula is this displayed $\perp$, it terminates successfully. 
    \item[\footnotesize(L$\to$).] If $S:\Gamma,\alpha\to\beta\To\Delta$ and the principal formula is this $\alpha\to\beta$, we recursive search for subgoals $S_1:\Gamma\To\Delta,\alpha$ and $S_2:\Gamma,\beta\To\Delta$ and terminates if both of them terminate successfully.
    \item[\footnotesize(R$\to$).] If $S:\Gamma\To\Delta,\alpha\to\beta$ and the principal formula is this $\alpha\to\beta$, we recursively search for subgoal $S_1: \Gamma,\alpha\To\Delta,\beta$ and terminates if the subgoal terminates successfully. 
    \item[\footnotesize(L$\forall$).] If $S:\Gamma,\forall x~\alpha\To\Delta$ and the principal formula is this $\forall x~\alpha$, we find some term $t$ and recursively search for $S_t:\Gamma,\forall x~\alpha,\alpha(x/t)\To\Delta$, where $\alpha(x/t)$ is obtained by replacing all free occurrence of $x$ with $t$.
    \item[\footnotesize(R$\exists$).] If $S:\Gamma\To\Delta,\exists x\;\beta$ and the principal formula is this $\exists x~\beta$, we find some term $t$ and recursively search for the subgoal $S_t:\Gamma\To\Delta, \beta(x/t), \exists x\;\beta$.  
    \item[\footnotesize(L$\exists$).] If $S:\Gamma,\exists x~\alpha\To\Delta$ and the principal formula is this $\exists x~\alpha$, we pick a fresh variable (i.e.~has no occurrence in $S$) $z$ and recursively search for the subgoal $S_z:\Gamma,\alpha(x/z)\To\Delta$. 
    \item[\footnotesize(R$\forall$).] If $S:\Gamma\To\Delta,\forall x~\beta$ and the principal formula is this $\forall x~\beta$, we pick a fresh variable (i.e.~has no occurrence in $S$) $z$ and recursively search for the subgoal $S_z:\Gamma\To\Delta,\beta(x/z)$.  
\end{description}

Note that the only non-determinism of the proof search procedure after we specify the principal formula $\psi$ is the term $t$ in (R$\exists$) and (L$\forall$): It does not contain any non-deterministic guess of intermediate subgoals thanks to the cut-free property. (For comparison, the proof-search interpretation of the cut rule is as follows: Given the selected goal $S:\Gamma\To\Delta$, we resolve $S$, guess a formula $\alpha$, and introduce two subgoals $S_1:\Gamma\To\Delta,\alpha$ and $S_2:\Gamma,\alpha\To\Delta$.)

\paragraph{Proof Search and Debate.} It is instructive to imagine the proof search procedure as the rule of a debate on the validity of the goal: we need to argue about the validity of the goal and defend the challenges from the opponent, who is skeptical about our claims. For simplicity, let us focus on quantifier rules (R$\exists$) and (R$\forall$), interpreted as follows. 

\inote{Not super clear what is going on in this debate in terms of the goal of the players and the rules...}

\begin{itemize}[itemsep=0pt]
    \item (R$\forall$): Now we need to argue that if $\Gamma$ holds, either a formula in $\Delta$ holds, or $\forall x~\beta$ holds. To prevent me from winning the debate, the opponent has to challenge the validity of $\forall x~\beta$ by giving a counter-example $z$ such that $\beta(x/z)$ does not hold. \inote{Why does the opponent have to challenge this?} To minimize my advantage, the opponent will not introduce any restriction on $z$, meaning that $z$ should be a fresh variable.
    \item (R$\exists$): Now we need to argue that if $\Gamma$ holds, either a formula in $\Delta$ holds, or $\exists x~\beta$ holds. We can propose some $t$ to witness $\exists x~\beta$ such that we only need to argue that at least one of $\Delta,\exists x~\beta,\beta(x/t)$ holds. This means that if we fail to argue that $\beta(x/t)$ holds, the knowledge we learned from the opponent (i.e., the counter-examples given by the opponent) can be used to propose a new $t'$ for $\exists x~\beta$. 
\end{itemize}
Note that the interpretation of (L$\exists$) and (L$\forall$) is similar to that of (R$\forall$) and (R$\exists$), respectively. 

Given this interpretation of the proof search procedure, roughly speaking, if $\varphi(x)$ is provable (i.e.~the proof search terminates successfully), the terms $t$ will (in some sense) witness the existential quantifiers in the conclusion, with the help of the counter-examples $z$ given by the opponent.   \inote{Is there a way to provide more intuition about this claim?}


\paragraph{Simple Case: Recovering KPT Witnessing.} We start with the simple case where $\varphi(x)$ is a $\Sigma^b_2$-formula, i.e., $\varphi(x)=\exists y_1~\forall x_1~\phi(x,x_1,y_1)$ for some quantifier-free formula $\phi$. As discussed above, the proof search procedure starts with the goal $S_0:\Gamma\To\varphi(x)$ for some finite $\Gamma\subseteq\calT$. Consider the principal formula chosen in the first step of the proof search procedure. 
\begin{enumerate}[itemsep=0pt]
    \item If some $\alpha\in\Gamma$ is selected as the principal formula, then the rule applied has to be one of (L$\to$) and (L$\forall$) by checking the form of all rules. \inote{Justify in a bit more detail or give an example for the previous claim.} In either case, we will introduce at most two subgoals of the form $\Gamma'\To\varphi(x)$, where $\Gamma'$ contains universal or quantifier-free formulas. For simplicity, we postpone the discussion of this situation and focus on the other case. 
    \item Otherwise, $\varphi(x)=\exists y_1~\forall x_1~\phi(x,x_1,y_1)$ is selected as the principal formula, then the rule applied has to be (R$\exists$). \inote{Again, explain why.} We will introduce a subgoal $S_1:\Gamma\To\varphi(x), \forall x_1~\phi(x,x_1,t_1)$ for some term $t_1(x)$. Intuitively, this means that we attempt to witness the outermost existential quantifier of $\varphi(x)$ by a term $t_1(x)$ (hence $\forall x_1~\phi(x,x_1,t_1(x))$ appears at the succedent). At the same time, we do not remove $\varphi(x)$ from the succedent, which means that if we cannot find a proof for $\forall x_1~\phi(x,x_1,t_1(x))$, we may go back to $\varphi(x)$ and propose a new term later. 
\end{enumerate} 

Suppose that, for instance, it is the second case, thus the subgoal we need to prove is $S_1:\Gamma\To\varphi(x), \forall x_1~\phi(x,x_1,t_1(x))$. As in the first step, we can choose the principal formula either in the antecedent or in the succedent, and we postpone the discussion of the former case. We argue (informally) that if we need to choose the principal formula in the succedent, choosing $\forall x_1~\phi(x,x_1,t_1(x))$ is \emph{preferable}, in the sense that we can always succeed by choosing $\forall x_1~\phi(x,x_1,t_1(x))$ here if it is possible for us to terminate successfully. Consider the interpretation of the proof search as a debate: when we apply (R$\forall$) with $\forall x_1~\phi(x,x_1,t_1(x))$ being principal, we force the opponent to challenge the validity of the the principal formula by providing a counter-example $z_1$, which gives us more information and thus makes it easier to search for the proof. As a result, we can apply (R$\forall$) now so that the goal becomes $S_2:\Gamma\To\varphi(x),\phi(x,z_1,t_1(x))$. 

Suppose that in the subsequent step, we, again, choose $\varphi(x)$ as the principal formula, so that the goal becomes 
\[
    S_3:\Gamma\To\varphi(x),\phi(x,z_1,t_1(x)),\forall x_1~\phi(x,x_1,t_2(x,z_1))
\]
for some term $t_2$, which can depend on both $x$ and $z_1$ (the counter-example for $\forall x_1~\phi(x,z_1,t_1(x))$). By the same argument as in the previous step, we should immediately apply (R$\forall$) so that the goal becomes 
\[
    S_4:\Gamma\To\varphi(x),\phi(x,z_1,t_1(x)),\phi(x,z_2,t_2(x,z_1))
\]
where $z_2$ is a fresh variable representing the counter-example of $\forall x_1~\phi(x,x_1,t_2(x,z_1))$. These two steps can repeat for arbitrarily (but constantly) many times \inote{Why constant?}, until we have terms $t_1,\dots,t_\ell$ and counter-examples $z_1,\dots,z_\ell$, the goal becomes 
\[
    S_{2\ell}:\Gamma\To\varphi(x),\phi(x,z_1,t_1(x)),\phi(x,z_2,t_2(x,z_1)),\dots,\phi(x,z_\ell,t_\ell(x,z_1,\dots,z_{\ell-1})),
\]
and we no longer need to propose new term $t$ for $\varphi$ to terminate the proof search. This means that even if we drop $\varphi(x)$ from the succedent, we can still terminate the proof search, which further means by the soundness of the proof search procedure that 
\[
\land\Gamma\to\phi(x,z_1,t_1(x))\lor \phi(x,z_2,t_2(x,z_1))\lor \dots\lor \phi(x,z_\ell,t_\ell(x,z_1,\dots,z_{\ell-1}))
\]
is a tautology. Since the formulas in $\Gamma\subseteq\calT$ hold in the standard model, we know that in the standard model, either $\phi(x,z_1,t_1(x))$ holds, or $\phi(x,z_2,t_2(x,z_1))$ holds, $\dots$, or $\phi(x,z_\ell,t_\ell(x,z_1,\dots,z_{\ell-1}))$ holds, meaning that $t_1,\dots,t_\ell$ computes a witness for $\exists y_1~\forall x_1~\phi(x,x_1,y_1)$ by learning from the counter-examples $z_1,\dots,z_\ell$. This recovers the KPT-witnessing theorem. 

\inote{Above, the meaning of ``if we drop $\varphi(x)$ from the succedent, we can still terminate the proof search'' is not clear.}

It remains to consider the case when, instead of choosing $\varphi(x)$ as the principal formula, we choose some $\alpha\in\Gamma$ in the first step, or choose the quantifier-free formula $\phi(x,x_1,t_1(x))$ in the third step, etc., in the proof search. The crucial observation is that in such cases, we will only apply one of (L$\forall$), (L$\to$), (Ax), (L$\perp$), and (R$\to$), and none of these rules can \emph{give} us counter-examples!\footnote{In particular, we will not apply (L$\exists$) since $\calT$ is a universal theory and there is no existential quantifier in $\Gamma$, and the existential quantifiers in the succedent will not be ``moved'' to the antecedent by (R$\to$) as long as $\varphi$ is explicitly written in the prenex normal form.} As the only non-determinism in the proof search is the term $t$ in (L$\forall$) and (R$\exists$) that involves the counter-examples, we can postpone all these rule applications until we finish proposing $t_1,t_2,\dots,t_\ell$. This completes the proof.  

\inote{Above, why can we postpone all these rule applications?}

\paragraph{Tree Exploration Game.} We now consider the general case where $\varphi(x)$ is a $\Sigma^b_i$ formula for any $i\ge 2$. For simplicity of presentation, we assume that $i=2k$ and $\varphi(x)$ is written explicitly as $\exists y_1~\forall x_1~\dots~\exists y_k~\forall x_k~\varphi(x,\vec x,\vec y)$. The proof search procedure starts with the goal $S_0:\Gamma\To\varphi(x)$ for some finite $\Gamma\subseteq\calT$. As discussed above, we will focus on the applications of (R$\exists$) and (R$\forall$) and ignore the applications of other rules. Furthermore, we apply the (R$\forall$) rule immediately when it is possible, since it will never make the proof search harder. 

Denote $\varphi[i]\eqdef\exists y_{i+1}~\forall x_{i+1}~\dots\exists y_k~\forall x_k~\phi(x,\vec x,\vec y)$, e.g., $\varphi[0]=\varphi$. In the first two steps of the proof search, we can only apply (R$\exists$) and then (R$\forall$), so that the goal becomes 
\[
S_1:\Gamma\To\varphi(x),\varphi[1](y_1/t_1(x),x_1/z_1)    
\] 
for some term $t_1$ and fresh variable $z_1$. Then we will have two choices: we can either choose $\varphi(x)$ or $\varphi[1](y_1/t_1(x),x_1/z_1)$ as the principal variable to apply (R$\exists$). Assume, for instance, we choose $\varphi[1](y_1/t_1(x),x_1/z_1)$ as the principal formula, then the goal becomes: 
\[
S_2:\Gamma\To\varphi(x),\varphi[1](y_1/t_1(x),x_1/z_1),\varphi[2](y_1/t_1(x),x_1/z_1,y_2/t_2(x,z_1),x_2/z_2)     
\]
for some term $t_2$ and fresh variable $z_2$. Here the proposed term $t_2$ can depend on both $x$ and the counter-example $z_1$ learned in the first two steps. After this step, we can choose any one of the three formulas as the principal formula. For instance, we choose $\varphi(x)$ and the goal becomes: 
\[
S_3:\Gamma\To\varphi(x),\varphi[1](y_1/t_1(x),x_1/z_1),\varphi[2](y_1/t_1(x),x_1/z_1,y_2/t_2(x,z_1),x_2/z_2),\varphi[1](y_1/t_3(z_1,z_2),x_1/z_3)
\]
for some term $t_3$ and fresh variable $z_3$. Then we can, again, choose a formula in the succedent, etc.

\begin{figure}
    \centering
    \begin{subfigure}{0.2\linewidth}
    \centering
    \begin{tikzpicture}[circle]
    \node (r) [draw] {1}
        child { 
            node (n1) [draw] {2} edge from parent [->]; 
        }
        child {
            node (n2) [] {};         
        };
        \path (r) -- (n1) node[midway,left] {\footnotesize$(y_1/t_1(x),x_1/z_1)$};
    \end{tikzpicture}
    \end{subfigure}
    ~
    \begin{subfigure}{0.25\linewidth}
        \centering
        \begin{tikzpicture}[circle]
        \node (r) [draw] {1}
            child { 
                node (n1) [draw] {2} edge from parent [->]
                child {
                    node (n3) [draw] {3} edge from parent [->];
                } 
            }
            child {
                node (n2) [] {};         
            };
            \path (r) -- (n1) node[midway,left] {\footnotesize$(y_1/t_1(x),x_1/z_1)$};
            \path (n1) -- (n3) node[midway,left] {\footnotesize$(y_2/t_2(x,z_1),x_2/z_2)$};
        \end{tikzpicture}
    \end{subfigure}
    ~
    \begin{subfigure}{0.4\linewidth}
        \centering
        \begin{tikzpicture}[circle]
        \node (r) [draw] {1}
            child { 
                node (n1) [draw] {2} edge from parent [->]
                child {
                    node (n3) [draw] {3} edge from parent [->];
                } 
            }
            child {
                node (n2) [draw] {4} edge from parent[->];
            };
            \path (r) -- (n1) node[midway,left] {\footnotesize$(y_1/t_1(x),x_1/z_1)$};
            \path (n1) -- (n3) node[midway,left] {\footnotesize$(y_2/t_2(x,z_1),x_2/z_2)$};
            \path (r) -- (n2) node[midway,right] {\footnotesize$(y_1/t_3(x,z_1,z_2),x_1/z_3)$};
        \end{tikzpicture}
    \end{subfigure}
    \caption{Tree structure of the succedent in this example.}\label{fig:tree-structure}
\end{figure}

\inote{Below, when explaining the pivotal observation, is there a way to provide more details and intuition?}

The pivotal observation here is that, during the applications of (R$\exists$) and (R$\forall$) as discussed above, the formulas in the succedent naturally form a tree structure, where each application of (R$\exists$) together with the subsequent (R$\forall$) creates a new node to the tree (see \Cref{fig:tree-structure}). Each node of depth $d$ (where the root is of depth $0$) corresponds to a substitution of free variables to $\varphi[i]$. Furthermore, if we substitute $x/n_0$ and $\vec z/\vec n$ on the tree by numbers $n_0,\vec n$ in $\bbN$, it becomes a finite upper part of the game tree of the \emph{evaluation game} of $\varphi(n_0)$ on $\bbN$, defined as follows: 
\begin{itemize}
    \item In the $i$-th step for $i\in[k]$, the \emph{truthifier} chooses a number $m_i\in\bbN$, then the falsifier chooses a number $n_i\in\bbN$. The truthifier wins if and only if $\phi(x/n_0,\vec y/\vec m, \vec x/\vec n)$ is true (in the standard model $\bbN$), where $\vec m=(m_1,\dots,m_k)$ and $\vec n=(n_1,\dots,n_k)$.  
\end{itemize} 
This motivates the definition of the \emph{tree exploration game} as follows: 
\begin{itemize}
    \item The game starts with the root being the only explored node in the game tree of the evaluation game. At each step, the \emph{truthifier} chooses an explored node $u$ and proposes some $m_i\in\bbN$ representing the move of the truthifier in the underlying evaluation game; the \emph{falsifier} then proposes $n_i\in\bbN$ as the response of the falsifier in the underlying evaluation game. After this step, the children of the $u$ corresponding to the move $(m_i,n_i)$ becomes explored. The truthifier wins if and only if a winning node in the game tree is explored. 
\end{itemize}
We note that here we define the evaluation game and tree exploration game on the standard model only for simplicity of presentation. The witnessing works for any model for $\calT$. 

Suppose that after applying (R$\exists$) and (R$\forall$) for $\ell=O(1)$ times (i.e.~after we branch the tree for $\ell$ times), we can terminate the proof search without further applications of (R$\exists$). This means that we can terminate the proof search successfully even if we remove all but the quantifier-free formulas in the succedent, or correspondingly, even if we remove all the nodes of depth $<k$. Let $\sigma_1,\sigma_2,\dots,\sigma_t$ be the substitutions to $\varphi[k]$ corresponding to the nodes of depth $k$. By the soundness of the proof search procedure, this means that 
\[
\land\Gamma\to \varphi[k](\sigma_1)\lor \varphi[k](\sigma_2)\lor\dots\lor \varphi[k](\sigma_t)    
\]
is a tautology. Since the formulas in $\Gamma\subseteq\calT$ hold in the standard model, we know that at least one of $\varphi[k](\sigma_1),\dots,\varphi[k](\sigma_t)$ is true in the standard model, i.e., at least one of them corresponds to a winning node of the evaluation game. This means that in the tree exploration game, if we explore the game tree as in the proof search procedure and propose the numbers $n_i$ according to the terms $t_1,t_2,\dots$, then no matter how the falsifier responds (i.e.~substituting numbers $m_i\in\bbN$ for the variables $z_i$), we will always reach a winning node of the evaluation game! 

By formalizing the argument above with an induction on the proof tree (or equivalently, the proof search procedure), we can extract a winning strategy for the exploration game from a proof (equivalently, a successfully terminated proof search). 


\subsection{Unprovability of strong complexity lower bounds}

XXX

\noindent \textbf{The Universal Theory $\UTpv^i$.}\\

\noindent \textbf{A Special Case of Game-Theoretic Witnessing: The Evaluation Game.}\\

\noindent \textbf{Witnessing Strong Complexity Lower Bounds.}\\

\noindent \textbf{X}

==> witnessing-general.tex <==
\subsection{Game-theoretic witnessing: Proof of \Cref{thm:witnessing-tree-exploration}} \label{sec:proof_game_theoretic_witnessing}

In this section, we provide a self-contained proof of \Cref{thm:witnessing-tree-exploration} using a Gentzen-style sequent calculus. We note that \Cref{thm:witnessing-tree-exploration} can also be established via model-theoretic methods (see a proof sketch in \cite{DBLP:journals/jsyml/BussKT14}), or by other proof-theoretic tools, such as the generalised Herbrand Theorem (see, e.g., \cite{buss1998handbook,mckinley2010sequent}) or the Midsequent Theorem (Gentzen's ``Sharpened Hauptsatz'', see, e.g., \cite[Section 5]{basic-proof-theory} and references therein) following essentially the same idea.\footnote{We thank an anonymous reviewer and J. Kraj\'{i}\v{c}ek for suggesting these alternative approaches.} 





\subsubsection{Overview}

Recall that we would like to extract computational information from a proof of a sentence in a bounded theory. Our argument relies on techniques from \emph{proof theory}, a discipline that investigates proofs as precise mathematical objects. In a bit more detail, we explore the structural properties of proofs in Gentzen's cut-free sequent calculus for (classical) first-order logic. We work with the related proof system $\GG$ defined in the classical textbook \cite{basic-proof-theory}. Here we only informally discuss the system $\GG$ and its connection to our witnessing theorem, leaving the formal definitions and arguments to \Cref{sec:witnessing-1}. 
 



Rather than dealing with formulas, the sequent calculus $\GG$ manipulates \emph{sequents} $\Gamma\To\Delta$, where $\Gamma$ (called the \emph{antecedent}) and $\Delta$ (called the \emph{succedent}) are finite multiset of formulas. The semantic interpretation of a sequent $\Gamma\To\Delta$ refers to $\land\Gamma\to\lor\Delta$, i.e., at least one of the formulas in $\Delta$ holds if all the formulas in $\Gamma$ hold. The system $\GG$ is known to be \emph{sound} and \emph{complete}, namely a sequent $\Gamma\To\Delta$ is valid (i.e.~$\land\Gamma\to\lor\Delta$ is true in all first-order structures) if and only if there is a derivation of $\Gamma\To\Delta$ from the rules and axioms of $\GG$. In particular, assuming that $\calT$ is a universal theory and $\forall x~\varphi(x)$ is a formula provable from $\calT$, we know by the compactness theorem (see \Cref{thm:compactness}) that there is a finite subset $\Gamma_\calT\subseteq\calT$ such that $\Gamma_\calT\vdash\varphi(x)$, which further means that the sequent $\Gamma_\calT\To\varphi(x)$ has a $\GG$-proof. Consequently, we aim to extract computational information from the $\GG$-proof of $\Gamma_\calT\To\varphi(x)$.

The most important feature that makes $\GG$ (and other variants of cut-free sequent calculus) useful in the extraction of information from proofs is that the $\GG$-proofs are \emph{highly structured}, in the sense that there is essentially no ``ad-hoc guess'' in $\GG$ when considering intermediate lemmas in a proof of a sentence. Concretely, $\GG$ does not offer rules such as the \emph{Modus Ponens} rule $\alpha,\alpha\to\beta\vdash\beta$ that makes the proof of $\beta$ dependent on a ``syntactically irrelevant'' guessed formula $\alpha$. In fact, each (non-axiom) rule of $\GG$ is uniquely determined by the outer-most connective or quantifier of a chosen occurrence of a formula (which is called the \emph{principal formula} of the rule) in the conclusion. The absence of ``ad-hoc guesses'' for intermediate formulas in a proof significantly simplifies the analysis of the $\GG$-proof of $\Gamma_\calT\To\varphi(x)$ via the syntactic structure of $\Gamma_\calT$ and $\varphi(x)$. We refer to \Cref{example:rules-g3c} for a concrete example. 

\begin{example}\label{example:rules-g3c}
    Consider the propositional rules (L$\to$) and (R$\to$) as an example:
    \[
    \frac{\Gamma\To\Delta,\alpha~~~~~~\Gamma,\beta\to\Delta}{\Gamma,\alpha\to\beta\To\Delta}~~(\text{L$\to$})~~~~~~~~~~\frac{\Gamma,\alpha\to\beta,\Delta}{\Gamma\To\alpha\to\beta,\Delta}~~(\text{R$\to$})    
    \]
    The principal formula in each of these rules is the displayed $\alpha\to\beta$ in the conclusion. As the name of the rule indicates, (L$\to$) (resp.~(R$\to$)) is uniquely determined when a formula with $\to$ as the outermost connective in the antecedent (resp.~succedent) of the conclusion is chosen as the principal formula. In other words, no other rule of the system $\GG$ is admissible once we fix this formula and consider its location in the sequent.
\end{example}

Since $\calT$ is a universal theory, every formula in $\Gamma_\calT$ is of the form $\forall\vec z~\beta(\vec z)$ for some quantifier-free formula $\beta$. Moreover, by a simple translation we can assume that $\varphi(x)$ is written in prenex normal form: 
\begin{equation} \nonumber
    \varphi(x)=\exists y_1~\forall x_1~\dots~\exists y_k~\forall x_k~\phi(x,x_1,\dots,x_k,y_1,\dots,y_k) \label{equ: def-of-varphi}    
\end{equation}
for some quantifier-free formula $\phi$. Consequently, one can show that the last rule application in the proof of $\Gamma_\calT\To\phi$ will be uniquely determined by the choice of the principal formula, which is either some $\forall\vec z\beta(\vec z)\in \Gamma_\calT$ or $\varphi(x)$. In both cases, we have control over the syntactic structure of the premise of the last rule application. We can then consider the second from the last rule application by looking at all the possible choices of the principal formula, and so on, until we reach the axioms employed in the proof. 

By a careful structural induction over the $\GG$-proof, we demonstrate that the applications of the \emph{quantifier rules} of $\GG$ (omitted in this brief overview) for principal formulas in the succedent have a correspondence to the tree exploration game. Through the applications of these rules and the fact that a (fixed finite) proof establishes the validity of the sentence $\forall x\,\varphi(x)$ in all first-order structures that satisfy $\calT$, we show how to extract a universal winning $\calL$-strategy of length $O(1)$ for the truthifier from the proof.

In the subsequent sections, we explain the approach in detail.


\subsubsection{A cut-free sequent calculus}
\label{sec:cut-free-g3c}
We assume familiarity with basic aspects of proof theory and Gentzen-style sequent calculi for first-order logic. We refer the reader to the standard textbook \citep{basic-proof-theory} for the necessary background.

Our main technical tool to prove the game-theoretic witnessing theorem is a cut-free sequent calculus for classical first-order logic known as $\GG$ (see Sections 3 and 4 of \cite{basic-proof-theory}).\footnote{To give some context, in \cite{basic-proof-theory} the system $\mathsf{G1c}$ is close to the original sequent calculus $\mathsf{LK}$ of Gentzen, $\mathsf{G2c}$ is a variant with weakening absorbed into the logical rules, and $\GG$ has both weakening and contraction absorbed into the rules and axioms.} We follow the notation and conventions from \cite{basic-proof-theory}, unless explicitly stated otherwise. %

For simplicity, we will work with the (complete) set $\{\perp,\to\}$ of connectives. Other Boolean connectives can be expressed using these in the usual way. For this set of connectives, the system $\GG$ contains the following rules (see \citep[Section 3.5]{basic-proof-theory}).\footnote{Restricting the rules of $\GG$ to our set of connectives can be done without loss of generality by the ``separation property'' of $\GG$ (see the first corollary in \citep[Section 4.2]{basic-proof-theory}).}\\


\noindent \textbf{Sequent Calculus $\bm{\GG}$:}\vspace{-0.3em}

\begin{multicols}{2}
\begin{prooftree}
    \AxiomC{}
    \LeftLabel{Ax:}
    \UnaryInfC{$\Gamma,P\To\Delta,P$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$\Gamma\To\Delta,\alpha$}
    \AxiomC{$\Gamma,\beta\To\Delta$}
    \LeftLabel{L$\to$:}
    \BinaryInfC{$\Gamma,\alpha\to\beta\To\Delta$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$\Gamma,\alpha(x/t),\forall x~\alpha(x)\To\Delta$}
    \LeftLabel{L$\forall$:}
    \UnaryInfC{$\Gamma,\forall x~\alpha(x)\To\Delta$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$\Gamma,\alpha(x/y)\To\Delta$}
    \LeftLabel{L$\exists$:}
    \UnaryInfC{$\Gamma,\exists x~\alpha(x)\To\Delta$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{}
    \LeftLabel{L$\perp$:}
    \UnaryInfC{$\Gamma,\perp\To\Delta$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$\Gamma,\alpha\To\Delta,\beta$}
    \LeftLabel{R$\to$:}
    \UnaryInfC{$\Gamma\To\Delta,\alpha\to\beta$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$\Gamma\To\Delta,\alpha(x/y)$}
    \LeftLabel{R$\forall$:}
    \UnaryInfC{$\Gamma\To\Delta,\forall x~\alpha(x)$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$\Gamma\To\Delta,\alpha(x/t),\exists x~\alpha(x)$}
    \LeftLabel{R$\exists$:}
    \UnaryInfC{$\Gamma\To\Delta,\exists x~\alpha(x)$}    
\end{prooftree}

\end{multicols}

\vspace{-0.2cm}


\paragraph{Notes.} Recall that in a sequent $\Sigma\To\Pi$ both $\Sigma$ and $\Pi$ are multisets of formulas. As usual, $\Sigma$ is called the \emph{antecedent} and  $\Pi$ is called the \emph{succedent}. In the rules above, $\alpha$ and $\beta$ are formulas. In the rule (Ax), $P$ is an atomic predicate, i.e., $P$ is of the form $R(t_1, \ldots, t_k)$, where $R$ is a relation symbol and $t_1, \ldots, t_k$ are arbitrary terms. The variable $y$ appearing in rules (R$\forall$) and (L$\exists$) has no free occurrences in the conclusion, i.e., in the formulas in $\Gamma \cup \Delta \cup \{\forall x~\alpha\}$ or $\Gamma \cup \Delta \cup \{\exists x~\alpha\}$. The formula denoted by $\alpha(x)$ can contain free variables besides $x$. A proof tree of a sequent $\Sigma\To\Pi$ is a tree of the applications of the eight rules, where the conclusion (root of the tree) is $\Sigma\To\Pi$ and the leaves have no premise (i.e., they are applications of (Ax) or (L$\perp$)). 

\paragraph{Naming convention.} Following the naming convention of \cite{basic-proof-theory}, for all the eight rules, we call the formula in the conclusion besides $\Gamma$ and $\Delta$ the \emph{principal formula}. The formulas in $\Gamma$ and $\Delta$ in both the premise and the conclusion are called \emph{side formulas}. The formulas in $\Gamma,\Delta$ in the conclusion of (Ax) and (L$\perp$) are called \emph{weak formulas}. The formulas in the premise that are neither side nor weak are called \emph{active formulas}; in particular, the formulas in the premises that are identical to the principal formulas (i.e.,~$\forall x~\alpha(x)$ in (L$\forall$) and $\exists x~\alpha(x)$ in (R$\exists$)) are called \emph{Kleene copies}. The variable $y$ in (R$\forall$) or (L$\exists$) is called the \emph{proper variable} of $\alpha$. 

\paragraph{Bounded variable renaming.} As in \cite{basic-proof-theory}, we identify the formulas that differ only by a renaming of the bounded variables in the rest of the section. Strictly speaking, this means that formulas appeared in the sequents are actually representing an equivalence class of the formulas up to a bounded variable renaming. Under this convention, we can have the completeness of $\GG$:

\begin{theorem}[Completeness of $\GG$ {\citep[Chapter 4]{basic-proof-theory}}]
    Let $\Gamma,\Delta$ be finite multiset of formulas. If $\bigwedge\Gamma\to\bigvee\Delta$ is a tautology, then $\Gamma\To\Delta$ is a provable sequent.
\end{theorem}

\paragraph{Dealing with Non-logical Axioms.} The sequent calculus $\GG$ defined above is for first-order logic without non-logical axioms and the axioms for equality. To deal with the theory $\Tpv^i$ that contains (infinitely many) non-logical axioms, we can simply use the compactness theorem of first-order logic. 

\begin{theorem}[Compactness Theorem for First-Order Logic]\label{thm:compactness}
    Let $\Gamma$ be a set of formulas, and $\varphi$ be a formula. Then $\Gamma\vdash\varphi$ if and only if there is a finite multiset $\Gamma_0$ of formulas in $\Gamma$ such that $\Gamma_0\vdash\varphi$. 
\end{theorem}

The compactness theorem and the completeness of $\GG$ imply that for every theory $\calT$, if $\calT\vdash\alpha$, then there exists a finite set $\Gamma$ of axioms in $\calT$ such that $\Gamma\To\alpha$ is a provable sequent. In particular, when $\calT$ is a universal theory, as in the statement of \Cref{thm:witnessing-tree-exploration}, we can assume w.l.o.g.~that the sentences in $\Gamma$ are \emph{explicitly} written in the form $\forall\vec x~\varphi(\vec x)$ for some quantifier-free formula $\varphi$. We will then extract a universal winning $\calL$-strategy from the proof tree of the sequent $\Gamma\To\alpha$.

\paragraph{Comparison with proof systems in previous works.} Many proof-theoretic results in bounded arithmetic utilize some systems of sequent calculus that contain restricted cut rules (see, e.g., the free-cut-free system in \cite{Buss} and anchored $\LK$ in \cite{cook_nguyen_2010}). Those systems are designed to treat the theories as a part of the proof system, while the system $\GG$ we use do not have this feature. 

\paragraph{Representation of bounded formulas.} To simplify the structure of the proof trees, we need to choose a canonical representation of bounded formulas. Let $\varphi(x)$ be a $\Sigma^b_k$-formula in prenex normal form (with bounded quantifiers). We define the following translation $[\cdot]_{\sf imp}$ that transforms a bounded formula in prenex normal form into a logically equivalent formula with only unbounded quantifiers:
\begin{itemize}[itemsep=0pt]
    \item If $\varphi(\vec x)$ is quantifier free, $[\varphi(\vec x)]_{\sf imp}\triangleq\varphi(\vec x)$. 
    \item If $\varphi(\vec x)=\forall y\le t(\vec x)~\phi(\vec x,y)$ and $[\phi]_{\sf imp}= Q_1 z_1~Q_2 z_2\dots Q_k z_k~\alpha(\vec x,y,\vec z)$, where $Q_i\in\{\forall,\exists\}$ for $i\in[k]$ and $\alpha$ is quantifier-free, then $[\varphi(\vec x)]_{\sf imp}\triangleq \forall y~Q_1 z_1~Q_2 z_2\dots Q_k z_k(y\le t(\vec x)\to \alpha(\vec x,y,\vec z))$.
    \item If $\varphi(\vec x)=\exists y\le t(\vec x)~\phi(\vec x,y)$ and $[\phi]_{\sf imp}= Q_1 z_1~Q_2 z_2\dots Q_k z_k~\alpha(\vec x,y,\vec z)$, where $Q_i\in\{\forall,\exists\}$ for $i\in[k]$ and $\alpha$ is quantifier-free, then $[\varphi(\vec x)]_{\sf imp}\triangleq \exists y~Q_1 z_1~Q_2 z_2\dots Q_k z_k(y\le t(\vec x)\land \alpha(\vec x,y,\vec z))$.\footnote{Note that a conjunction $\alpha \land \beta$ can be written as $(\alpha \to (\beta \to \bot)) \to \bot$. As mentioned above, when discussing provability in $\GG$ we will assume w.l.o.g.~that the quantifier-free part of $[\varphi]_{\sf imp}$ is written using connectives from $\{\to, \bot\}$.}
\end{itemize}
We say a formula $\varphi$ is \emph{implicitly bounded} if there is a bounded formula $\psi$ in prenex normal form such that $\varphi=[\psi]_{\sf imp}$.

\begin{proposition}
For every bounded formula $\varphi(x)$ in prenex normal form (with bounded quantifiers), $[\varphi(x)]_{\sf imp}$ is logically equivalent to $\varphi(x)$. 
\end{proposition}

\begin{proof}
This follows from a simple induction with the logical equivalence $\alpha \star (Q x~\beta)\equiv Q x~(\alpha\star\beta)$ for any $\star\in\{\to,\land\}$ and $Q\in\{\forall,\exists\}$ when $x$ has no free occurrence in $\alpha$. 
\end{proof}


\subsubsection{Structural transformations of the proof tree}

Let $\varphi(x)=\exists y_1~\forall x_1\dots \exists y_k~\forall x_k~\phi(x,\vec x,\vec y)$ be an implicitly bounded formula with exactly one free variable $x$ for quantifier-free $\phi$. We denote the sub-formula of $\varphi$ starting from the $(i+1)$-th existential quantifier $\exists y_{i+1}~\forall x_{i+1}\dots \exists y_k~\forall x_k~\phi(x, \vec x,\vec y)$ as $\varphi[i]$ (e.g. $\varphi=\varphi[0]$).\footnote{Strictly speaking, we define $\varphi[i]$ as the sub-formula starting from the $(i+1)$-th existential quantifier, where the bounded variables $y_1,\dots,y_j$ and $x_1,\dots,x_j$ are replaced by fresh free variables. Here, we slightly abuse the notation to call the fresh variables still by $y_1,\dots,y_j$ and $x_1,\dots,x_j$. The readers should keep in mind that a renaming has been done here to avoid naming conflicts between these bounded variables and other free variables.} Let $\Gamma$ be a finite multiset of universal sentences written explicitly in the form $\forall\vec x~\beta(\vec x)$ for some quantifier-free formula $\beta(x)$, i.e., it contains only universal quantifiers and no propositional connective occurs outside of a (universal) quantifier. We will prove some structural lemmas for a proof tree of $\Gamma\To\forall x~\varphi(x)$.

\begin{lemma}\label{lmm:universal-to-free-var} Under these assumptions, 
    $\Gamma\To\forall x~\varphi(x)$ is provable if and only if $\Gamma\To\varphi(x)$ is provable.
\end{lemma}

\begin{proof}
    Since $\Gamma$ contains no free variables, the (if) side is proved by directly applying (R$\forall$). The (only if) side follows by the admissibility of the inversion rule of (R$\forall$) (see, e.g., Proposition 3.5.4 of \cite{basic-proof-theory}). 
\end{proof}

\begin{definition}
    A formula is called \emph{simple} if it is either quantifier free or a universal formula. A set or multiset of formulas is called \emph{simple} if all its formulas are simple.
\end{definition}

\begin{lemma}\label{lmm:subformula}
    A formula occurs in a proof tree of $\Gamma\To\varphi(x)$ is either simple or a substitution to $\varphi[i]$ for some $i\in[0,k]$. Moreover, any antecedent formula must be simple, and any succedent formula is either quantifier-free or a substitution to $\varphi[i]$ for $i\in[0,k]$. 
\end{lemma}

\begin{proof}
    Assume that it is not the case. Find any lowest (i.e. closest to the root) step $\frac{\Sigma'\To\Pi'}{\Sigma\To\Pi}$ such that a formula in $\Sigma',\Pi'$ violates the property above. By checking the eight rules of $\GG$ it's easy to find a contradiction.
\end{proof}

\paragraph{Replacing (R$\to$) with (R$\to_c$).} For technical reasons, we will replace (R$\to$) with the following rule (R$\to_c$) with built-in contradction, i.e., we introduce an additional Kleene copy $\alpha\to\beta$ in the succedent of the premise.

\begin{prooftree}
\AxiomC{$\Gamma,\alpha\To\Delta,\beta,\alpha\to\beta$}
\RightLabel{(R$\to_c$).}
\UnaryInfC{$\Gamma\To\Delta,\alpha\to\beta$}
\end{prooftree}

\begin{lemma}\label{lmm:right-weakening}
    Let $\Gamma,\Delta$ be arbitrary multisets of formulas. Assume that there is a $\GG$ proof tree $T$ of $\Gamma\To\Delta$. Then there is a proof tree $T'$ of $\Gamma\To\Delta$ that has no (R$\to$) and may contain (R$\to_c$).   
\end{lemma}

\begin{proof}
We perform induction on the number of the applications of (R$\to$) in the proof tree. Assume that there is at least one application of (R$\to$). Let $(X)$ be an arbitrary application of (R$\to$). We will replace $(X)$ to be an application of (R$\to_c$) by adding $\alpha\to\beta$ to the succedent of every sequent within the sub-tree rooted at $(X)$. It is easy to see that the new proof tree is also a valid proof tree, where $\alpha\to\beta$ is either a side formula or a weak formula inside the sub-tree above $(X)$. Moreover, the number of (R$\to$) is decreased by $1$ so we can complete the proof by the induction hypothesis. 
\end{proof}

\paragraph{Limiting the applications of (R$\exists$) and (R$\forall$).} We also need to perform some proof transformation to ``pair'' the applications of (R$\exists$) and (R$\forall$): we want to have a one-to-one correspondence between the applications of (R$\exists$) and (R$\forall$) such that the application of (R$\exists$) immediately follows from its corresponding application of (R$\forall$). Intuitively, this is possible since the succedent formula of the conclusion is highly structured and the antecedent contains only simple formulas. 

\begin{definition}
    An application ($X$) of (R$\forall$) is said to be \emph{limited} if it is followed by an application of (R$\exists$) such that the principal formula of the (R$\forall$) is the same as the active formula of the (R$\exists$). It is said to be \emph{unlimited} if it is not limited.

    An application ($Y$) of (R$\exists$) is said to be \emph{limited} if it immediately follows a limited application of (R$\forall$). It is said to be \emph{unlimited} if it is not limited.
\end{definition}

\begin{definition}
    Let $T$ be a proof tree, $x$ be a variable, and $t$ be a term. The substitution $T(x/t)$ is defined as the tree where all the free occurrence of $x$ are replaced by $t$.
\end{definition}

\begin{lemma}[$\beta$-substitution]\label{lmm:beta}
    If $T$ is a proof tree of $\Gamma\To\Delta$ in $\GG+(\text{R}\to_c)$, then $T(x/t)$ is a proof tree of $\Gamma(x/t)\To\Delta(x/t)$, provided that $t$ contains no free occurrence of $x$ and free variables in $T,\Gamma,\Delta$.
\end{lemma}

\begin{proof}
    Induction on the proof tree (see, e.g., Lemma 3.5.2 of \cite{basic-proof-theory}).
\end{proof}

\begin{lemma}\label{lmm:no-limited-ru}
    If $\Gamma\To\varphi(x)$ is provable, then there is a proof tree $T$ of $\Gamma\To\varphi(x)$ such that: (1) $T$ has no $(R\to)$ and may contain $(R\to_c)$; (2) $T$ has no unlimited application of (R$\forall$).  
\end{lemma}

\begin{proof}
    Let $T$ be a proof tree of $\Gamma\To\varphi(x)$. By \Cref{lmm:right-weakening}, we can assume without loss of generality that $T$ contains no (R$\to$) and may contain (R$\to_c$). We will then construct a new proof tree $T'$ satisfies the property (2) above by removing all the unlimited applications of (R$\forall$). Let 
    \begin{prooftree}
        \AxiomC{$\Gamma\To\Delta,\alpha(x/w)$}
        \RightLabel{($X$)}
        \UnaryInfC{$\Gamma\To\Delta,\forall x~\alpha(x)$}
    \end{prooftree}
    be an uppermost (i.e. farthest to the root) invalid application of (R$\forall$). By Lemma \ref{lmm:subformula} we know that $\alpha$ is a substitution of $\varphi[i]$ for some $i\in[1,k]$, and $x$ is $x_{i}$. It is easy to see that on the path from ($X$) to the root, there must be an application of (R$\exists$) with active formula $\forall x~\alpha(x)$, such that the premise of this (R$\exists$) is not derived immediately from an application of (R$\forall$) with $\forall x~\alpha(x)$ being principal.\footnote{Assume not, this $\forall x~\alpha(x)$ can only be a side formula or an active formula on the path from ($X$) to the root. It cannot be an active formula since no rule other than (R$\exists$) can has universally quantified active formula on the succedent (recall that we assume all the propositional connectives appear within quantifiers). Therefore it must be side formulas, meaning that it must appear in the succedent of the conclusion, which is impossible.}

    Find an uppermost application of (R$\exists$) satisfying the property above. It is of form 
    \begin{prooftree}
        \AxiomC{$\Sigma\To\Pi,\forall x_{i}~\alpha(x_i),\exists y_{i}~\forall x_{i}~\alpha'(x_i,y_i)$}
        \RightLabel{($Y$)}
        \UnaryInfC{$\Sigma\To\Pi,\exists y_{i}~\forall x_{i}~\alpha'(x_i,y_i)$}
    \end{prooftree}
    Note that $x_i$ is $x$ and $\alpha$ is a substitution of $\alpha'$ on the existentially bounded variable $y_i$. Find all the unlimited rule applications $(X_1),(X_2),\dots,(X_m)$ of (R$\forall$) above ($Y$) such that for all $j\in[m]$, (1) $\forall x_i~\alpha(x_i)$ is principal in $(X_j)$, and (2) there is no rule application of (R$\forall$) on the path from $(X_j)$ to $(Y)$ that satisfies (1). Clearly $m\ge 1$ since $(X)$ satisfies (1). 
    
    \begin{itemize}
    \item We add a limited application of (R$\forall$) immediately above (Y), as follows. 
    \begin{prooftree}
        \AxiomC{$\Sigma\To\Pi,\alpha(x_i/z),\exists y_{i}~\forall x_{i}~\alpha'(x_i,y_i)$}
        \RightLabel{($X'$)}
        \UnaryInfC{$\Sigma\To\Pi,\forall x_{i}~\alpha(x_i),\exists y_{i}~\forall x_{i}~\alpha'(x_i,y_i)$}
        \RightLabel{($Y$)}
        \UnaryInfC{$\Sigma\To\Pi,\exists y_{i}~\forall x_{i}~\alpha'(x_i,y_i)$}
    \end{prooftree}
    where $z$ is a fresh variable that has no free occurrence in the proof tree. This new formula $\alpha(x_i/z)$ is added as a side or weak formula into all the sequents in the subtree rooted at ($Y$) except for the parts above ($X_j$) for some $j\in[1,m]$.
    \item For each $(X_j)$ with premise $\Gamma_j\To\Delta_j,\phi(x/w_j)$, we apply Lemma \ref{lmm:beta} to obtain a proof tree of $\Gamma_j\To\Delta_j,\alpha(x_i/z)$ ($(\alpha(x_i/y_j)(y_j/z)=\alpha(x_i/z)$). We then remove the application ($X_j$) directly and link this new proof tree back. This is possible since $\alpha(x_i/z)$ has been available as a side formula. 
    \end{itemize}
    By doing this we can remove at least one unlimited application of (R$\forall$). The lemma then follows by a simple induction. 
\end{proof}

For convenience, we will use (R$\exists\forall$) to denote a pair of adjacent limited (R$\forall$) and (R$\exists$), and regard (R$\exists\forall$) as a single rule of the following form in a proof tree with only limited applications of (R$\forall$) and (R$\exists$). 
\begin{prooftree}
    \AxiomC{$\Gamma\To\Delta,\alpha(y/t, x/z),\exists y~\forall x~\alpha(y,x)$}
    \LeftLabel{R$\exists\forall$:}
    \UnaryInfC{$\Gamma\To\Delta,\exists y~\forall x~\alpha(y,x)$} 
\end{prooftree}
where $t$ is a term, and $z$ is a fresh variable without free occurrence in $\Gamma,\Delta$, and $\forall x~\alpha(y/t,x)$. We call $z$ the \emph{proper variable} in the application of this rule.

\paragraph{Canonical Proofs.} Now we show that if $\Gamma\To\varphi(x)$ is provable, then it has a well-structured proof. We need to use the following $\beta$-substitution lemma for $\GG+(\text{R}\exists\forall)+(\text{R}\to_c)$. Similar to previous definition, we define $T(x/t)$ be the proof tree obtained from $T$, where all free occurrences of $x$ are replaced by $t$. It can be easily proved by structural induction on the proof tree $T$. 

\begin{lemma}[$\beta$-substitution for $\GG+(\text{R}\exists\forall)+(\text{R}\to_c)$]\label{lmm: beta on new}
    Assume that $T$ is a proof tree of $\Gamma\To\Delta$ with $\GG+(\text{R}\exists\forall)+(\text{R}\to_c)$, then $T(x/t)$ is a proof tree of $\Gamma(x/t)\To\Delta(x/t)$, provided that $t$ contains no free occurrence of $x$ and free variables in $T,\Gamma,\Delta$.
\end{lemma}



\begin{definition}
    A proof tree $T$ for $\Gamma\To\varphi(x)$ is said to be \emph{canonical} if it satisfies the following three properties:
    \begin{enumerate}[itemsep=0pt] 
    \item $T$ does not contain (R$\forall$), (R$\exists$), (R$\to$), and (L$\exists$). It may contain (R$\exists\forall$) and (R$\to_c$). 
    \item Each sequent in $T$ is of form $\Gamma\To\Phi,\Theta$ where $\Gamma$ contains only simple formulas, $\Phi$ contains substitutions to $\varphi[i]$ for some $i\in[0,k]$, and $\Theta$ contains quantifier-free formulas.
    \item Each free variable occurs in $T$ except for $x$ is introduced as the proper variable in an application of (R$\exists\forall$) for the universal quantifier.
    \end{enumerate}
\end{definition}

\begin{theorem}\label{thm:normalized-proof}
    Let $\varphi(x)=\exists y_1~\forall x_1\dots \exists y_k~\forall x_k~\phi(x,\vec x,\vec y)$ be an implicitly bounded formula with exactly one free variable $x$ for quantifier-free $\phi$, and $\Gamma$ be a set of universal formulas written explicitly in the form $\forall\vec x~\beta(\vec x)$ for some quantifier-free $\beta(\vec x)$. If $\Gamma\To\varphi(x)$ is provable, then there is a canonical proof tree for $\Gamma\To\varphi(x)$. 
\end{theorem}
\begin{proof}
We first apply Lemma \ref{lmm:no-limited-ru} to remove all the unlimited applications of (R$\forall$) and replace (R$\to$) by (R$\to_c$). We add a useless limited (R$\forall$) above every unlimited application of (R$\exists$) to make it limited (the active formula of this (R$\forall$) is added as a side or weak formula in the sequents above). Then we replace all the pairs of adjacent applications of (R$\forall$) and (R$\exists$) by (R$\exists\forall$). 

The second property can be proved similar to Lemma \ref{lmm:subformula}. The only thing to check is that the new rules (R$\to_c$) and (R$\exists\forall$) maintain the subformula property. 

For the third property, we only need to consider (R$\exists\forall$) and (L$\forall$) where a term $t$ (which may contain new variables) is introduced for the existential and universal quantifiers, respectively. For every such application, if the term $t$ contains other free variables, we apply Lemma \ref{lmm: beta on new} to substitute all other free variables to be $0$. 
\end{proof}


\newcommand{\tikzmark}[2]{\tikz[overlay,remember picture] \node[baseline] (#1) {#2};}

\begin{figure}
    \centering
    \begin{adjustbox}{minipage=\linewidth,scale=0.58,left,frame}
    \vspace{0.25cm}
    \begin{prooftree}
    \AxiomC{}
    \RightLabel{(Ax)}
    \UnaryInfC{$P(x,g(x,z_1)),\forall z~\varphi(x,z),\forall x~\forall z~\varphi(x,z),Q(f(x),z_1),Q(g(x,z_1),z_2)\To Q(f(x),z_1)\to P(x,f(x)),P(x,f(x)),\psi(x),P(x,g(x,z_1)),Q(g(x,z_1),z_2)\to P(x,g(x,z_1))$}
    \RightLabel{(R$\to_c$)}
    \UnaryInfC{$P(x,g(x,z_1)),\forall z~\varphi(x,z),\forall x~\forall z~\varphi(x,z),Q(f(x),z_1)\To Q(f(x),z_1)\to P(x,f(x)),P(x,f(x)),\psi(x),Q(g(x,z_1),z_2)\to P(x,g(x,z_1))$}
    \RightLabel{$(\text{R}\exists\forall)_2$}
    \UnaryInfC{$\stackrel{\displaystyle P(x,g(x,z_1)),\forall z~\varphi(x,z),\forall x~\forall z~\varphi(x,z),Q(f(x),z_1)\To Q(f(x),z_1)\to P(x,f(x)),P(x,f(x)),\psi(x)}{\tikzmark{p1}{}}$}
    \end{prooftree}
    \vspace{0.3cm}
    
    \begin{prooftree}
    \AxiomC{}
    \RightLabel{(Ax)}
    \UnaryInfC{$\forall z~\varphi(x,z),\forall x~\forall z~\varphi(x,z),Q(f(x),z_1)\To Q(f(x),z_1),Q(f(x),z_1)\to P(x,f(x)),P(x,f(x)),\psi(x)$}
    \AxiomC{\tikzmark{p2}{$\dots$}}
    \RightLabel{(L$\to$)}
    \BinaryInfC{$Q(f(x),z_1)\to P(x,g(x,z_1)),\forall z~\varphi(x,z),\forall x~\forall z~\varphi(x,z),Q(f(x),z_1)\To P(x,f(x)),Q(f(x),z_1)\to P(x,f(x)),\psi(x)$}
    \RightLabel{(L$\forall$)}
    \UnaryInfC{$\forall z~\varphi(x,z),\forall x~\forall z~\varphi(x,z),Q(f(x),z_1)\To P(x,f(x)),Q(f(x),z_1)\to P(x,f(x)),\psi(x)$}
    \RightLabel{(L$\forall$)}
    \UnaryInfC{$\forall x~\forall z~\varphi(x,z),Q(f(x),z_1)\To P(x,f(x)),Q(f(x),z_1)\to P(x,f(x)),\psi(x)$}
    \RightLabel{(R$\to_c$)}
    \UnaryInfC{$\forall x~\forall z~\varphi(x,z) \To Q(f(x),z_1)\to P(x,f(x)),\psi(x)$}
    \RightLabel{$(\text{R}\exists\forall)_1$}
    \UnaryInfC{$\forall x~\forall z~\varphi(x,z)\To\psi(x)$}
    \end{prooftree}
    \begin{tikzpicture}[overlay,remember picture]
    \draw[->] (p2.north) .. controls +(up:15mm) and +(down:15mm) ..  (p1.south);
    \end{tikzpicture}
    \end{adjustbox}
    \caption{A canonical proof tree of $\forall x~\forall z~\varphi(x,z)\To\psi(x)$, where $\varphi(x,z)\triangleq Q(f(x),z)\to P(x,g(x,z))$, $\psi(x)\triangleq\exists y~\forall z~(Q(y,z)\to P(x,y))$.}
    \label{fig:g3c-example}
\end{figure}


\subsubsection{Unbounded tree exploration games}

Due to technical reasons, we need to define unbounded variants of the tree exploration games and partial game trees. Let $\varphi(x)=\exists y_1~\forall x_1\dots \exists y_k~\forall x_k~\phi(x,\vec x,\vec y)$ be an implicitly bounded $\calL$-formula as discussed above and $(\calM=(\calD,\calI),n_0)$ be a board. An \emph{unbounded partial game tree} for $\varphi$ on the board $(\calM,n_0)$ is defined as a finite rooted tree on which each edge is labeled with a pair $(m,n)\in\calD\times\calD$ of elements. The \emph{unbounded tree exploration game} starting from an unbounded partial game tree $T$ of $\varphi$ is defined as follows. In each round, the truthifier chooses a node $u$ on the tree and specifies a number $m\in\calD$; the falsifier then specifies a number $n\in\calD$; after this round, a child of $u$ is added to the tree by an edge labeled $(m,n)$. The truthifier wins if and only if there is a node on the tree such that the pairs on the path from the root to the node form a satisfying assignment of $\phi(x/n_0,\vec x,\vec y)$ within $\calM$, where the truthifier's moves are for $\vec y$ and the falsifier's moves are for $\vec x$. In particular, the unbounded tree exploration game of $\varphi$ is defined as the game starting from a tree with only the root.

An $\calL$-strategy of the truthifier of length $\ell\in\bbN$ and initial tree size $d$ is a sequence $$\tau=\left<p_1,r_1,p_2,r_2,\dots,p_\ell,r_\ell\right>\,,$$  where $p_i$ is an $\calL$-term and $r_i\in\bbN$ such that $1\le r_i<d+i$. Let $(\calM,n_0)$ be a board and $T$ be an unbounded partial game tree on the board with $d$ nodes numbered $1,2,\dots,d$. The game-theoretic strategy for the unbounded tree exploration game starting from $T$ induced by $\tau$ is the following strategy: 
\begin{itemize}
    \item In the $i$-th move, the truthifier introduces a node numbered $d+i$ as a child of the node $r_i$, and chooses the element $v_i\triangleq p_i^{\calM}(n_0,T,\Gamma)\in\calM$, where $\Gamma$ describes the moves of previous rounds (including $v_1,\dots,v_{i-1}$ and the falsifier's moves). 
\end{itemize}
A length-$\ell$ $\calL$-strategy is said to be a universal winning strategy if the truthifier playing the induced game-theoretic strategy wins within $\ell$ moves against any strategy of the falsifier on any board $(\calM, n_0)$. 

\begin{lemma}\label{lmm:strategy-unbounded-to-bounded}
    Let $\calT$ be a bounded theory over the language $\calL$ that is closed under if-then-else. If there is an $O(1)$-length $\calL$-strategy that is a universal winning strategy of the truthifier for the unbounded tree exploration game of $\varphi = [\psi]_{\sf imp}$, then there is an $O(1)$-length $\calL$-strategy that is a universal winning strategy of the truthifier for the tree exploration game of $\psi$. 
\end{lemma}
\begin{proof}
Assume that $\tau=\left<p_1,r_1,p_2,r_2,\dots,p_\ell,r_\ell\right>$ is a universal winning $\calL$-strategy of length $\ell\in\bbN$ for the unbounded tree exploration game. Let $p_i'(x,\Gamma)$ be the term defined as follows:

\begin{enumerate}[topsep=0pt, itemsep=0pt]
    \item Parse $\Gamma=(m_1,n_1,m_2,n_2,\dots,m_{i-1},n_{i-1})$ as the moves in previous rounds. 
    \item Define $\Gamma_0$ to be the empty list and $\hat \Gamma_{j+1}$ to be 
    \[
    \hat \Gamma_{j+1}=\begin{cases}
    \hat \Gamma_{j};(m_{j+1},n_{j+1}) & \text{if } m_{j+1}=p_{j+1}(n_0,\hat \Gamma_j) \\ 
    \hat \Gamma_{j};(p_{j+1}(n_0,\hat \Gamma_j),0) & \text{otherwise}
    \end{cases}
    \]
    \item Output $0$ if $p_i(n_0,\hat \Gamma_{i-1})$ is not a valid move (i.e., it violates the inequality for the bounded variable); and output $p_i(n_0,\hat \Gamma_{i-1})$ otherwise.  
\end{enumerate}
Note that such $p_i'$ always exists as $\calT$ is closed under if-then-else. We now argue that the $\calL$-quasi-strategy $\tau'\triangleq \left<p_1',r_1,p_2',r_2,\dots,p_\ell',r_\ell\right>$ is indeed a universal winning $\calL$-strategy for the tree exploration game of $\psi$. Intuitively, $\tau'$ is the following $\calL$-quasi-strategy: it simulates $\tau$ if it gives a valid move; otherwise, it simply outputs $0$ and ``forgets'' the response of the falsifier, pretending that in this round it simulates $\tau$ and the falsifier's response were $0$. 

By the definition of $p_i'$ it is easy to see that $\tau'$ is an $\calL$-strategy for the tree exploration game of $\psi$, since it will never output an invalid move. Towards a contradiction we assume that it is not a universal winning strategy. In such case, there exist a board $(\calM,n_0)$ and a strategy $\tau_\ttf'$ for the falsifier that prevents the truthifier from winning within $\ell$ rounds on the board against the truthifier playing the induced strategy of $\tau'$. We now construct a strategy $\tau_\ttf$ of the falsifier for the unbounded tree exploration game of $\varphi$ on the board $(\calM,n_0)$ that prevents $\tau$ from winning within $\ell$ rounds and thus leads to a contradiction.

\begin{itemize}[topsep=0pt]
    \item Assume that the moves of $\tau_\ttf'$ against $\tau'$ is $n_1',n_2',\dots,n_\ell'$. In the $i$-th move, if the truthifier's move is an invalid move in the (bounded) tree exploration game (i.e., it violates the inequality for the bounded variable), the falsifier chooses $n_i\triangleq 0$; otherwise the falsifier chooses $n_i\triangleq n_i'$.   
\end{itemize}
It is easy to check that against this strategy of the falsifier, $\tau$ cannot win within $\ell$ rounds. This is because the transcript of $\tau_\ttf$ vs $\tau$ is exactly the lists $\hat \Gamma$ in the definition of $\tau'$; and since $\tau'$ cannot win against $\tau'_\ttf$ within $\ell$ rounds, $\tau$ also cannot win against $\tau_\ttf$ within $\ell$ rounds.  
\end{proof}

This lemma shows that to obtain a winning strategy of the tree exploration game, we only need to extract a winning strategy of the unbounded tree exploration game from a $\GG$ proof tree. In practice, this means that we do not need to treat bounded quantifiers in a special way.

\subsubsection{Partial game trees from sequents}

\newfunc{\pr}{path}
\newfunc{\pgt}{pgt}

Let $T$ be a canonical proof tree of $\Gamma\To\varphi(x)$. An \emph{$\calL$-term partial game tree} $T_\calL$ of $\varphi(x)$ is a rooted tree that satisfies the following properties. Assume that the nodes are $v_1,v_2,v_3,\dots,v_{\ell}$, where $v_1$ is the root, $p_i$ be the parent of $v_i$, and $e_i$ be the edge connecting $v_i$ and $p_i$ for $2\le i\le \ell$. Let $\pr(i)$ denote the edges on the path from $v_i$ to the root. Then: 
\begin{enumerate}[itemsep=0pt]
\item Each node $v_i$ is marked as a number $o_i\in\{1,\dots,\ell\}$ such that $o_i>o_{p_i}$, i.e., it is a topological order. This $o_i$ indicates the order of the introduction of the nodes in the partial game tree. 
\item Each edge $e_i$ is associated with a pair $(q_i,z_i)$, where $z_i$ is a variable and $q_i$ is an $\calL$-term. The variables $\{z_i\}$ are pairwise distinct, and the term $q_i$ only contains $x$ and the variables $z_j$ for $o_j< o_i$ as free variables.
\end{enumerate}
We also denote it by $T_\calL(x,z_1,z_2,\dots,z_\ell)$ to explicitly display the free variables.

Let $(\calM=(\calD,\calI),n_0)$ be a board. Given an $\calL$-term partial game tree $T_\calL$ and an assignment for the free variables on the tree: $n_0\in\calD$ for $x$ and $n_1,n_2,\dots,n_{\ell}\in\calD$ for the variables $z_1,z_2,\dots,z_{\ell}$ on the tree with concrete numbers, we can construct a corresponding \emph{unbounded} partial game tree by replacing $z_i$ with $n_i\in\calD$ and $q_i$ with $q_i^\calM(x/n_0,z_1/n_1,\dots,z_\ell/n_\ell)\in\calD$ for every $i\in[\ell]$. We denote this unbounded partial game tree as $T_\calL(x/n_0,z_1/n_1,\dots,z_\ell/n_\ell)$. 

We will define a translation $[\cdot]_{\pgt}$ that maps a sequent in a canonical proof tree $T$ of $\Gamma\To\varphi(x)$ to a $\calL$-term partial game tree.\footnote{Strictly speaking, the translation $[\cdot]_{\pgt}$ is defined over the occurrences of the sequents in the proof tree $T$. In particular, two occurrences of the same sequent may be translated to different partial game trees. Here (and below), we slightly abuse the notation to say $[\Gamma\To\Psi]_\pgt$ for a sequent $\Gamma\To\Psi$, when the occurrence of $\Gamma\To\Psi$ that we are referring to is clear in the context.} To gain some intuition, it is instructive to image the (canonical) proof tree as formed in a proof search procedure, that is, from the root to the leaves. The substitutions of $\varphi[i]$ in the succedent are introduced as the active formulas when we apply (R$\forall\exists$). At the same time, the principal formula in the conclusion occurs as the Kleene copy in the premise. For every sequent $\Gamma\To\Phi,\Theta$ as described above, the formulas in $\Phi$ were introduced in the proof search as a tree structure, where the initial formula $\varphi(x)$ at the root of the proof tree is the root, and the active formula introduced when applying (R$\forall\exists$) is a child of the principal formula (which becomes the Kleene copy in the premise) of this rule application. This tree structure naturally corresponds to an $\calL$-term partial game tree $T_G=[\Gamma\To\Phi,\Theta]_{\pgt}$, where the proper variables occur as $z_j$ in $T_G$ and the witnessing terms occur as $q_j$ in $T_G$.  




\newcommand{\obphi}{\mathsf{Sub}(\varphi)}

Formally, we defined the set of formulas \emph{obtained from substitutions of $\varphi[\cdot]$}, denoted by $\obphi$, as follows.\footnote{Strictly speaking, $\obphi$ should be a set of occurrences of formulas in the sequent instead of a set of formulas. Here (and below), we slightly abuse the notation to say that a formula is in $\obphi$, which actually means that the occurrence of the formula is in $\obphi$, when the occurrence is clear in the context.} A formula $\psi$ in the succedent of the canonical proof tree is in $\obphi$ if one of the following conditions hold: 
\begin{enumerate}[topsep=0.5em,itemsep=0em]
    \item The sequent containing $\psi$ is the conclusion and $\psi$ is $\varphi(x)$; 
    \item In the rule application with the sequent containing $\psi$ being the premise, $\psi$ is a side formula, and its counterpart in the conclusion is in $\obphi$;
    \item The sequent containing $\psi$ is the premise of a rule application of (R$\to_c$), $\psi$ is the Kleene copy, and the principal formula is in $\obphi$; 
    \item The sequent containing $\psi$ is the premise of a rule application of $(\text{R}\exists\forall)$, and $\psi$ is one of the two active formulas. 
\end{enumerate}
We can then write each sequent in the proof tree in the form $\Sigma\To\Pi,\Delta$, where $\Pi$ contains all the formulas in $\obphi$. It then follows from \Cref{lmm:subformula} that $\Delta$ contains only quantifier-free formulas.\footnote{Recall that the conclusion of the proof tree is $\Gamma\To\varphi(x)$, where $\Gamma$ contains universal sentences written explicitly in the form $\forall\vec z~\beta$ for some quantifier-free $\beta$. A formula $\alpha$ in the proof tree that is not in $\obphi$ is necessarily a sub-formula of some $\forall\vec z~\beta\in\Gamma$. As it appears in the succedent, on the path from it to the root there must be an application of (L$\to$) that ``carries'' it from the antecedent to the succedent. Since all the propositional connectives appears within the quantifier-free $\beta$, this formula $\alpha$ has to be quantifier-free.}

Now we define the translation by induction on the depth (i.e., the distance to the root) of the sequent $\Sigma\To\Pi,\Delta$ we want to translate within $T$. We will maintain the following properties during this recursive definition. 
\begin{itemize} 
\item\textbf{(Structure of Formulas in $\Pi$.)} Let $\Sigma\To\Pi,\Delta$ be a sequent in $T$ where $\Pi$ contains formulas in $\obphi$ and $\Delta$ contains quantifier-free formulas. For all $\alpha\in\Pi$, there is an $i\in[0,k]$ such that  
\[
\alpha=\exists y_{i+1}~\forall x_{i+1}\dots\exists y_k~\forall x_k~\phi(x,x_1/z_1,\dots,x_{i}/z_{i},y_1/q_1,\dots,y_{i}/q_{i}),
\] 
where $q_j$ is an $\calL$-term with no free variables except for $x$ and the free variables on the $\calL$-term partial game tree corresponding to the parent of this sequent (if it has a parent).
\item\textbf{(Formulas in $\Pi$ $\sim$ Nodes in Partial Game Tree).} For each sequent $\Sigma\To\Pi,\Delta$ in $T$ as described above, there is a one-to-one correspondence between the formulas $\alpha\in\Pi$ and the nodes $v\in[\Sigma\To\Pi,\Delta]_\pgt$. Let $\alpha\in\Pi$ be a formula of the form  
\[
\alpha=\exists y_{i+1}~\forall x_{i+1}\dots\exists y_k~\forall x_k~\phi(x,x_1/z_{j_1},\dots,x_{i}/z_{j_{i}},y_1/q_{j_1},\dots,y_{i}/q_{j_{i}}).
\] 
Then the edges on the path from the root to the node $v$ corresponding to $\alpha$ is associated with the pairs 
\[
(q_{j_1},z_{j_1}),(q_{j_2},z_{j_2}),\dots,(q_{j_{i-1}},z_{j_{i-1}}).
\]
\end{itemize}

Let $\Sigma\To\Pi,\Delta$ be a sequent in $T$ such that $\Pi$ contains formulas in $\obphi$ and $\Delta$ contains quantifier-free formulas.
\begin{itemize}
    \item If the depth is $0$, (i.e., we are at the root of the proof tree), we know that $\Delta=\varnothing$ and $\Pi=\{\varphi(x)\}$. We define $[\Sigma\To\Pi,\Delta]_{\pgt}$ as a $\calL$-term partial game tree with only the root.
    \item Otherwise we assume that the parent of the sequent is $\Sigma'\To\Pi',\Delta'$, where $\Pi'$ contains formulas in $\obphi$ and $\Delta'$ contains quantifier-free formulas. We consider which rule is applied to derive $\Sigma'\To\Pi',\Delta'$ from $\Sigma\To\Pi,\Delta$ (and another premise, if (L$\to$) is applied). There are the following possibilities: (L$\to$), (R$\to_c$), (L$\forall$), and (R$\exists\forall$).
\begin{enumerate}
    \item If the rule applied is one of (L$\to$), (R$\to_c$), and (L$\forall$), we know that $\Pi=\Pi'$, and we define $[\Sigma\To\Pi,\Delta]_\pgt\triangleq[\Sigma'\To\Pi',\Delta']_\pgt$. 
    \item If the rule applied is (R$\exists\forall$) with $\exists y_i~\forall x_i~\alpha(x_i,y_i)$ being principal, we know that $\Pi=\Pi'\cup\{\alpha(x_i/z,y_i/t)\}$ for some fresh variable $z$ and term $t$. By the definition of canonical proof tree and the invariant, we know that $t$ has no free variables except for $x$ and free variables in $\Sigma',\Pi',\Delta'$, which further means that $t$ has no free variables except for $x$ and the free variables in $[\Sigma'\To\Pi',\Delta']_\pgt$. 
    
    Let $T'_\pgt\triangleq[\Sigma'\To\Pi',\Delta']_\pgt$ be a partial game tree with $\ell$ nodes (including the root). Let $v\in T'_\pgt$ be the node corresponding to the formula $\exists y_i~\forall x_i~\alpha(x_i,y_i)\in\Pi'$, as promised in the induction hypothesis. We add a child of $v$ labeled $\ell+1$ that is connected to $v$ with an edge associated with the pair $(t,z)$. This child corresponds to the active formula $\alpha(x_i/z,y_i/t)\in\Gamma\setminus\Gamma'$, whereas the correspondence between other nodes and formulas are induced from the correspondence in $T'_\pgt$. (Note that the formulas in $\Pi'$ appears as side formulas or the Kleene copy in $\Pi$.) It's easy to verify that the two properties for the induction is satisfied and the new tree is still a valid $\calL$-term partial game tree.
\end{enumerate}
\end{itemize}

\begin{example}
For instance, consider the canonical proof tree of the sequent $\forall x~\forall z~(Q(f(x),z)\to P(x,g(x,z)))\To\exists y~\forall z~(Q(y,z)\to P(x,y))$ in \Cref{fig:g3c-example}. The $\calL$-term partial game tree corresponding to the sequent on the root is a tree with only the root; the game trees corresponding to the premises of $(\text{R}\exists\forall)_1$ and $(\text{R}\exists\forall)_2$ are shown in \Cref{fig:pgt-ref1} and \Cref{fig:pgt-ref2}, respectively. Node 1, Node 2, and Node 3 correspond to the following substitutions of $\exists y~\forall z~(Q(y,z)\to P(x,y))$ in the proof tree:  
\begin{align*}
\text{Node 1:}~~~&\exists y~\forall z~(Q(y,z)\to P(x,y)). \\ 
\text{Node 2:}~~~&Q(f(x),z_1)\to P(x,f(x)). \\ 
\text{Node 3:}~~~&Q(g(x,z_1),z_2)\to P(x,g(x,z_1)).
\end{align*}
The partial game trees corresponding to the other sequents in the proof tree are inherited from the partial game trees of their parents. 
\end{example}

\begin{figure}[htb]
    \begin{subfigure}{0.45\linewidth}
    \centering
    \begin{tikzpicture}[circle]
    \node (r) [draw] {1}
        child { 
            node (n1) [draw] {2} edge from parent [->]; 
        }
        child {
            node (n2) [] {};         
        };
        \path (r) -- (n1) node[midway,left] {$(f(x),z_1)$};
        \path (r) -- (n2) node[midway,right] {$\color{white}(g(x,z_1),z_2)$};
    \end{tikzpicture}
    \caption{PGT of the premise of $(\text{R}\exists\forall)_1$.}\label{fig:pgt-ref1}
    \end{subfigure}
    ~
    \begin{subfigure}{0.45\linewidth}
    \centering
    \begin{tikzpicture}[circle]
    \node (r') [draw] {1}
        child { 
            node (n1') [draw] {2} edge from parent [->]; 
        }
        child {
            node (n2') [draw] {3} edge from parent [->];
        };
        \path (r') -- (n1') node[midway,left] {$(f(x),z_1)$};
        \path (r') -- (n2') node[midway,right] {$(g(x,z_1),z_2)$};
    \end{tikzpicture}
    \caption{PGT of the premise of $(\text{R}\exists\forall)_2$.}\label{fig:pgt-ref2}
    \end{subfigure}
    \caption{Partial game trees corresponding to sequents in the proof tree in \Cref{fig:g3c-example}.}
\end{figure}



\subsubsection{Completing the argument: Winning strategies from proofs}

\begin{definition} 
Let $\tau=\left<p_1,r_1,p_2,r_2,\dots,p_{\ell},r_{\ell}\right>$ and $\tau'=\left<p_1',r_1',p_2',r_2',\dots,p_{\ell'}',r_{\ell'}'\right>$ be two $\calL$-term strategies with initial tree size $d$. We define the concatenation of the two strategies as 
\[
\tau;\tau'\triangleq\left<p_1,r_1,p_2,r_2,\dots,p_\ell,r_\ell,p_1',r_1',p_2',r_2',\dots,p_{\ell'}',r_{\ell'}'\right>. 
\]
Note that $\tau;\tau'$ is an $\calL$-term strategy with length $\ell+\ell'$ and initial tree size $d$. 
\end{definition}

\begin{lemma}\label{lmm:extract-strategy-from-proofs}
    Let $T$ be a canonical proof tree of $\Gamma\To\varphi(x)$, $\Sigma\To\Pi,\Delta$ be a sequent in $T$ (where $\Pi$ contains formulas in $\obphi$ and $\Delta$ contains quantifier-free formulas), and $T_G(x,z_1,z_2,\dots,z_d)\triangleq[\Sigma\To\Pi,\Delta]_\pgt$. There is an $O(1)$ length $\calL$-term strategy $\tau$ with initial tree size $d+1$ such that the following holds:
    \begin{itemize}[topsep=2pt,itemsep=0pt]
    \item \textbf{(Correctness).} Let $(\calM,n_0)$ be a board and $\sigma$ be an assignment of free variables in this $\Sigma\To\Pi,\Delta$ such that $\sigma(x)=n_0$. If in the model $\calM$ and with the assignment $\sigma$ to free variables, every formula in $\Sigma$ is true and every formula in $\Delta$ is false, the induced game-theoretic strategy of $\tau$ is a winning strategy for the unbounded tree exploration game starting from $T_G(x/n_0,z_1/\sigma(z_1),z_2/\sigma(z_2),\dots,z_d/\sigma(z_d))$.
    \item \textbf{(Extraction).} There is a polynomial-time algorithm that outputs the strategy for every sequent in $T$ given the canonical proof tree $T$ as input. 
    \end{itemize}
\end{lemma}

\begin{proof}
    Let $\Sigma\To\Pi, \Delta$ be a sequent in $\calT$, we prove that if this lemma holds for the premise(s) of this $\Sigma\To\Pi,\Delta$, then it also holds for this $\Sigma\To\Pi,\Delta$. The lemma then follows from a structural induction on $T$. Consider the rule application on this $\Sigma\To\Pi,\Delta$. 
    \begin{description}
    \item[Case 1.] If it is an application of (Ax), we consider the following two cases. 
    \begin{description}
    \item[Case 1.1.] Assume that the principal formula $P\notin\obphi$, i.e., the sequent is of form $\Sigma',P\To\Pi,\Delta',P$ for some atomic predicate $P$, where $\Sigma=\Sigma',P$ and $\Delta=\Delta',P$. Then for every board $(\calM,n_0)$ and assignment $\sigma$ for free variables in $\Sigma\To\Pi,\Delta$, in the model $\calM$ and with the assignment $\sigma$, it is impossible for all the formulas in $\Sigma$ to be true and all the formulas in $\Pi$ to be false, since $P\in\Sigma\cap\Pi$.
    \item[Case 1.2.] Otherwise, the principal formula $P\in\obphi$, i.e., the sequent is of form $\Sigma',P\To\Pi',\Delta,P$, where $\Sigma=\Sigma',P$ and $\Delta=\Delta',P$. Let $T_G\triangleq[\Sigma\To\Pi,\Delta]_\pgt$. Let $(M,n_0)$ be a board and $\sigma$ be an assignment of free variables in $\Sigma\To\Pi,\Delta$ such that $\sigma(x)=n_0$. In the model $\calM$ and with the assignment $\sigma$ to free variables, if all the formulas in $\Sigma$ are true, then $P\in\Sigma$ is true, meaning that the node in $T_G$ corresponding to $P\in\Pi$ is a winning node of the evaluation game of $\varphi$. In such case, a trivial strategy that does nothing is a winning strategy.  
    \end{description}
    \item[Case 2.] If it is an application of (L$\perp$), the sequent is of form $\Sigma',\perp\To\Pi,\Delta$. Similar to Case 1, it is impossible for all the formulas in $\Sigma$ to be true, since $\perp\in\Sigma$. 
    \item[Case 3.] If it is an application of (L$\to$), it is of form 
    \begin{prooftree}
    \AxiomC{$\Sigma'\To\Pi,\Delta,\alpha$}
    \AxiomC{$\Sigma',\beta\To\Pi,\Delta$}
    \BinaryInfC{$\Sigma',\alpha\to\beta\To\Pi,\Delta$}
    \end{prooftree}
    where $\Sigma=\Sigma',\alpha\to\beta$. Let $T_G\triangleq [\Sigma'\To\Pi,\Delta,\alpha]_{\pgt}=[\Sigma',\beta\To\Pi,\Delta]_\pgt=[\Sigma\To\Pi,\Delta]_{\pgt}$. The formula $\alpha\to\beta$ is simple. By the induction hypothesis, we know that there are $\calL$-strategies $\tau_1$ for $\Sigma'\To\Pi,\Delta,\alpha$ and $\tau_2$ for $\Sigma',\beta\To\Pi,\Delta$ satisfying this lemma. We know prove that $\tau_1;\tau_2$ is the desired strategy for this $\Sigma\To\Pi,\Delta$. Let $(\calM,n_0)$ be a board and $\sigma$ be an assignment of free variables such that $\sigma(x)=n_0$. If in the model $\calM$ and with the assignment $\sigma$ to free variables, all formulas in $\Sigma=\Sigma',\alpha\to\beta$ are true and all formulas in $\Delta$ are false, since $(\alpha\to\beta)\in\Sigma$ either $\alpha$ is false or $\beta$ is true. We can see from the induction hypothesis that: In the former case, $\tau_1$ will be a winning strategy for the unbounded tree exploration game starting from $T_G(x/n_0,z_1/\sigma(z_1),\dots,z_\ell/\sigma(z_\ell))$; in the latter case, $\tau_2$ will be a winning strategy for the same game. As a result, $\tau_1;\tau_2$ is always a winning strategy for the unbounded tree exploration game starting from $T_G(x/n_0,z_1/\sigma(z_1),\dots,z_\ell/\sigma(z_\ell))$.
    \item[Case 4.] If it is an application of (R$\to_c$), consider the following two cases.
    \begin{description}
    \item[Case 4.1.] Assume that the principal formula is not in $\obphi$. Then the rule applications is of form 
    \begin{prooftree}
    \AxiomC{$\Sigma,\alpha\To\Pi,\Delta',\beta,\alpha\to\beta$}
    \UnaryInfC{$\Sigma\To\Pi,\Delta',\alpha\to\beta$}
    \end{prooftree}
    where $\Delta=\Delta',\beta$. By the definition, we know that $\beta$ in the premise is not in $\obphi$. Let $T_G\triangleq[\Sigma,\alpha\To\Pi,\Delta',\beta]_\pgt=[\Sigma\To\Pi,\Delta]_\pgt$. Similar to Case 3, we can see the $\calL$-term strategy for the premise from the induction hypothesis is indeed the required $\calL$-term strategy for $\Sigma\To\Pi,\Delta$, because in any model and for any assignment to free variables, if $\alpha\to\beta$ is false, then $\alpha$ is true and $\beta$ is false. 
    \item[Case 4.2.] Now we assume that the principal formula is in $\obphi$. It is of form 
    \begin{prooftree}
    \AxiomC{$\Sigma,\alpha\To\Pi',\Delta,\beta,\alpha\to\beta$}
    \UnaryInfC{$\Sigma\To\Pi',\Delta,\alpha\to\beta$}
    \end{prooftree}
    where $\Pi=\Pi',\alpha\to\beta$. Let $T_G\triangleq [\Sigma\To\Pi,\Delta]_\pgt=[\Sigma,\alpha\To\Pi',\Delta,\beta,\alpha\to\beta]_\pgt$. We claim that the $\calL$-term strategy for the premise from the induction hypothesis is also the required $\calL$-term strategy for $\Sigma\To\Pi,\Delta$. Let $(\calM,n_0)$ be a board and $\sigma$ be an assignment of free variables in $\Sigma\To\Pi,\Delta$ such that $\sigma(x)=n_0$. Assume that in the model $\calM$ and with the assignment $\sigma$ to free variables, all the formulas in $\Sigma$ are true and all the formulas in $\Pi$ are false. Consider the following two cases: 
    \begin{enumerate}
        \item If $\alpha\to\beta$ is true, then the node corresponding to $\alpha\to\beta$ in $T_G$ is a winning node for the truthifier, which means that the truthifier wins the game regardless of its further moves. 
        \item Otherwise, $\alpha$ is true and $\beta$ is false. In such case, we can see from the induction hypothesis that the strategy from the premise will win in the tree exploration game starting from $T_G(x/n_0,z_1/\sigma(z_1),\dots,z_\ell/\sigma(z_\ell))$ on the board $(\calM,n_0)$. 
    \end{enumerate}
    As a result, the strategy from the premise is always a winning strategy. 
    \end{description}
    
    \item[Case 5.] If it is an application of (L$\forall$), it is of form 
    \begin{prooftree}
    \AxiomC{$\Sigma',\alpha(x/t)\To\Pi,\Delta$} 
    \UnaryInfC{$\Sigma',\forall x~\alpha(x)\To\Pi,\Delta$}
    \end{prooftree}
    where $\Sigma=\Sigma',\forall x~\alpha(x)$. Similar to Case 3 and Case 4, we can see that the $\calL$-term strategy for the premise from the induction hypothesis is indeed the required $\calL$-term for $\Sigma\To\Pi,\Delta$, since in any model and for any assignment to free variables, if $\forall x~\alpha(x)$ is true, then $\alpha(x/t)$ is true. 
    \item[Case 6.] If it is an application of (R$\exists\forall$), it is of form 
    \begin{prooftree}
    \AxiomC{$\Sigma\To\Pi',\Delta,\alpha(x/z,y/t),\exists y~\forall x~\alpha(y,x)$}
    \UnaryInfC{$\Sigma\To\Pi',\Delta,\exists y~\forall x~\alpha(y,x)$} 
    \end{prooftree}
    where $\Pi=\Pi',\exists y~\forall x~\alpha(y,x)$ and $\exists y~\forall x~\alpha(y,x)\in\obphi$, Let 
    \begin{align*}
    &T_G(z_1,z_2,\dots,z_{d-1})\triangleq[\Sigma\To\Pi,\Delta]_\pgt, \\ 
    &T_G'(z_1,z_2,\dots,z_{d-1},z)\triangleq[\Sigma\To\Pi',\Delta,\alpha(x/z,y/t),\exists y~\forall x~\alpha(y,x)]_\pgt,
    \end{align*}
    where $d$ is the number of nodes in $T_G$. Let $v_i$ be the node corresponding to $\alpha(x/z,y/t)$ in $T_G'$. Assume that $\exists y~\forall x~\alpha(y,x)$ corresponds to $v_j$ in $T_G$. By the induction hypothesis, there is a strategy $\tau_1=\left<p_1,r_1,p_2,r_2,\dots,p_\ell,r_\ell\right>$ for the premise that satisfies the lemma. We now show that the strategy $\tau = \left<t,j,p_1,r_1,p_2,r_2,\dots,p_\ell,r_\ell\right>$, which means (intuitively) that the truthifier will choose the node $v_j$ and add a number $t$ in the first round and then follow $\tau_1$, is the required $\calL$-term strategy for $\Sigma\To\Pi,\Delta$. 

    
    Let $(\calM,n_0)$ be a board and $\sigma$ been an assignment of free variables in $\Sigma\To\Pi,\Delta$ such that $\sigma(x)=n_0$. Assume that in the model $\calM$ with the assignment $\sigma$ to free variables, all the formulas in $\Sigma$ are true and all the formulas in $\Delta$ are false. We need to prove that the induced game-theoretic strategy of $\tau$ is a winning strategy of the unbounded tree exploration game starting from $T_G(x/n_0,z_1/\sigma(z_1),\dots,z_\ell/\sigma(z_\ell))$. According to the definition of $\tau$, the truthifier will choose $v_j\in T_G$ (i.e., the node corresponding to $\exists y~\forall x~\alpha(y,x)$) and a number $t^\calM$. Assume that the falsifier chooses $n_1\in\calM$ in its move. Let  $\sigma_1\triangleq\sigma\cup\{z/n_1\}$ be an assignment of free variables in the premise. 
    
    In the model $\calM$ and with the assignment $\sigma_1$, for the premise of this application of (R$\exists\forall$), all the formulas in the antecedent are true and all the formulas that are not in $\obphi$ in the succedent are false. Therefore by the induction hypothesis, the induced game-theoretic strategy $\tau_1$ is a winning strategy for the unbounded tree exploration game starting from $T_G'$ in the model $\calM$ and with the assignment $\sigma_1$. Since $\tau$ starts to simulate $\tau_1$ from the second step, the induced game-theoretic strategy of $\tau$ will also win.  
    \end{description}
    Note that although we do not explicitly discuss the extraction property, it is easy to verify that we can extract the strategy inductively using the proof above.
\end{proof}

\begin{reminder}[\Cref{thm:witnessing-tree-exploration}]
    Let $\calT$ be a universal bounded theory  with vocabulary $\calL$ that is closed under if-then-else. Let $\varphi$ be a bounded $\calL$-formula  of the form
    \begin{align*}
    \varphi(x)~\triangleq~&\exists y_1\le t_1(x)~\forall x_1\le s_1(x,y_1)~\exists y_2\le t_2(x,y_1,x_1)\dots \forall x_{k-1}\le s_{k-1}(x,y_1,x_1,\dots,y_{k-1})\\
  ~&\exists y_k\le t_k(x,y_1,x_1,\dots,y_{k-1}, x_{k-1})~\forall x_{k}\le s_k(x,y_1,x_1,\dots,y_{k})~\phi(x,x_1,\dots,x_k, y_1,\dots,y_k),
\end{align*}
where $\phi(x, \vec{x}, \vec{y})$ is a quantifier-free $\calL$-formula. Then $\calT\vdash\forall x~\varphi(x)$ if and only if there is a universal winning $\calL$-strategy of length $O(1)$ for the truthifier in the corresponding tree exploration game of $\varphi(x)$. 
\end{reminder}

\begin{proof}
    (If). Assume that $\calT\nvdash\forall x~\varphi(x)$. Then by the completeness theorem there is a model $\calM=(\calD,\calI)$ and $n_0\in\calD$ such that $\varphi^\calM(n_0)$ is false, which further means that there is a winning strategy of the falsifier in the evaluation game of $\varphi(x)$ on the broad $(\calM,n_0)$. Consider the strategy of the falsifier in the tree exploration game that simply simulates this winning strategy, i.e., after the truthifier adds a node and specifies an element on the edge, the falsifier treats the path from the root to this node as a partial transcript of the evaluation game and chooses an element according to the strategy of the evaluation game. It is clear that the truthifier cannot reach a winning node, thus it does not have a universal winning $\calL$-strategy of the tree exploration game.  
    
    (Only If). Let $\calL,\calT$ and $\varphi$ be defined as above. Suppose that $\calT\vdash \forall x~\varphi(x)$. By Lemma \ref{lmm:universal-to-free-var} and Theorem \ref{thm:normalized-proof}, there is a canonical proof tree for $\calT\vdash\varphi(x)$. By applying Lemma \ref{lmm:extract-strategy-from-proofs} and considering the root of the proof tree, there is an $O(1)$-length $\calL$-strategy $\tau$ for the unbounded tree exploration game of $\varphi(x)$. Finally, we can obtain an $O(1)$-length universal winning $\calL$-strategy $\tau$ for the tree exploration game of $\varphi(x)$ by Lemma \ref{lmm:strategy-unbounded-to-bounded}.
\end{proof}
    
\ignore{
    Let $\Gamma_i$ be the game board after the $i$-th round consisting of prefixes of transcripts of the evaluation games for $\varphi(m_0)$\footnote{That is, a sequence of numbers $(m_0,n_1,m_1,n_2,m_2,\dots,n_j,m_j)$ such that $n_l\le t_l(m_0,n_1,m_1,\dots,m_{l-1})$ and $m_l\le s_l(m_0,n_1,m_1,\dots,n_l)$.}, and $\Gamma_0=\{(m_0)\}$ be the game board at the beginning. In the $i$-th step, the truthifier will choose an $(m_0,n_1,m_1,\dots,n_j,m_j)\in\Gamma_{i-1}$ and a number $n_{j+1}\le t_{j+1}(m_0,n_1,m_1,\dots,m_{j})$; the falsifier will choose an $m_{j+1}\le s_{j+1}(m_0,n_1,m_1,\dots,m_j)$; and the board will be updated as $\Gamma_i\triangleq\Gamma_{i-1}\cup\{(m_0,n_1,m_1,\dots,n_{j+1},m_{j+1})\}$. The truthifier \emph{wins after the $i$-th round} if there is a complete game transcript $\func{trs}\in\Gamma_i$ (of length $2k+1$) on which the truthifier wins the evaluation game. 
}

\ignore{
    \begin{corollary}
    Any $\TF\Sigma_i$ problem provably total in $\Tpv^j$ can be solvable in $\P^{\Sigma_{j-1}^p}$ for all $j\ge 2$. Any $\TF\Sigma_i$ problem provably total in $\Tpv^1$ can be solvable in $\P^\NP$. In particular, any $\TF\NP$ problem provably total can be solvable in $\P$.
    \end{corollary}
    
    \begin{proof}
    ($j=1$ and $i>1$). Let $L$ be a $\TF\Sigma_i$ problem provable in $\Tpv$, say $L$ is defined by the $\Sigma_i^b$ sentence $\exists y_1\forall x_1\exists y_2\forall x_2\dots Qz\varphi(x_0,\vec x,\vec y)$ ($Q\in\{\exists,\forall\}$). Then by Theorem \ref{thm:witnessing-general}, there is an $\ell\in\bbN$ and $\ell$ polynomial-time strategies, such that for all strategy for the falsifier (i.e. the player to witness the universal quantifiers), if we play the evaluation game for $\ell$ times and give the transcripts of the previous games to the truthifier as ancillary information, the truthifier will win in at least one round. Now consider this specific strategy for falsifier: \begin{enumerate}
        \item In the $i$-th round of the evaluation game, if there is an $x$ that witnesses the universal quantifier (i.e. a winning move), then the falsifier chooses the lexicographical minimal $x$ that witnesses the the universal quantifier.
        \item Otherwise, the falsifier simply chooses $0$.
    \end{enumerate}
    According to the discussion above, we know that the truthifier will win at least one of the $\ell$ games against this specific strategy. In such case, the first move of the truthifier in at least one of the $\ell$ games should be a correct answer to the $\TF\Sigma_i$ search problem $L$. Now we describe a $\P^\NP$ algorithm solving $L$. 
\begin{enumerate}
    \item For $i=1,2,\dots,\ell$, we simulate the $\ell$ games, where the $k$-th game is given as the transcripts of the first $k-1$ games. 
    \item In the $k$-th game, we use the $\NP$ oracle and the search-to-decision reduction for SAT to find out the lexicographical minimal strategy for the falsifier to win the game. If such strategy does not exist, then the first move of the truthifier is the answer of the $\TF\Sigma_i$ problem. Otherwise, we can obtain the lexicographical minimal answer of the falsifier, which is given the $k+1,k+2,\dots,\ell$ games.   
\end{enumerate}
    Therefore in at least one of the $\ell$ games the falsifier will not find any answer, which means we can obtain a correct answer of the original $\TF\Sigma_i$ problem. 
    
    ($j=1$ and $i=1$). The result immediately follows from the standard witnessing theorem. 
    
    ($j\ge 2$). For each true $\Pi_j^b$ sentence, we introduce a $\TF\Sigma_{j-1}$ computable function symbol to turn it into a universal sentence. Then we roughly follow the case ($j=1$ and $i>1$). The only difference is that we obtain from the proof $\P^{\TF\Sigma_{j-1}}$ strategies instead of $\P$ strategies. Since the SAT of $\P^{\TF\Sigma_{j-1}}$ algorithm is in $\P^{\Sigma_{j-1}^p}$,\footnote{For any $\P^{\TF\Sigma_{j-1}}$ algorithm $A(x,y)$, the SAT problem $\exists y A(x,y)$ for it can be solved in $\P^{\Sigma^p_{j-1}}$ as follows: given input $x$, universally guess an $y$ and a computation history of $A(x,y)$, then verify the correctness of it with a $\Pi^p_{j-2}$ algorithm.} we can finally resolve the original $\TF\Sigma_{i}$ problem with a $\P^{\Sigma_{j-1}^p}$ algorithm.
    \end{proof}
}


